On Equivalence and Uniformisation Problems for Finite Transducers

Transductions are binary relations of finite words. For rational transductions, i.e., transductions defined by finite transducers, the inclusion, equivalence and sequential uniformisation problems are known to be undecidable. In this paper, we investigate stronger variants of inclusion, equivalence and sequential uniformisation, based on a general notion of transducer resynchronisation, and show their decidability. We also investigate the classes of finite-valued rational transductions and deterministic rational transductions, which are known to have a decidable equivalence problem. We show that sequential uniformisation is also decidable for them.

==> On Equivalence and Uniformisation Problems for Finite Transducers/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}
We have introduced the notion of resynchronisers, which are
transformations for synchronisations of transductions. The decision
problems of inclusion, equivalence, and sequential uniformisation, which
are undecidable for general rational transductions, become decidable
modulo rational resynchronisers. Furthermore, we have shown that it is
sufficient to consider $k$-delay resynchronisers in the context of
these decision problems. We have  analysed two subclasses of
transducers, finite-valued transducers and deterministic
transducers. For both classes, sequential uniformisation is decidable, and the
existence of a sequential uniformiser implies the existence of a
sequential $k$-uniformiser. Additionally, for finite-valued transducers $k$-inclusion is shown to be complete.
One interesting open question is the problem of deciding for a
transducer whether it admits a sequential $k$-uniformiser for some $k$. 

==> On Equivalence and Uniformisation Problems for Finite Transducers/decision.tex <==
\vspace{2mm}
\noindent\textbf{Decision problems for transducers modulo
  resynchronisers} Let $\Sigma$ be an alphabet, $\sync$ be a resynchroniser over
$(\inouta)^*$, and $\tra_1,\tra_2$ be two transducers over $\Sigma$.  
We say that $\tra_1$ is \emph{included in $\tra_2$ modulo $\sync$} (or
\emph{$\sync$-included}), denoted by $\tra_1\subseteq_\sync \tra_2$, if 
$\lang{\tra_1} \subseteq \sync(\lang{\tra_2})$. We say that $\tra_1$ is \emph{equivalent to
  $\tra_2$ modulo $\sync$} (or \emph{$\sync$-equivalent}), denoted by
$\tra_1 \equiv_\sync \tra_2$, if $\tra_1 \subseteq_\sync \tra_2$ and $\tra_2\subseteq_\sync
\tra_1$. For a fixed synchroniser $\sync$, the \emph{$\sync$-inclusion
(resp. $\sync$-equivalence) problem} asks, given two transducers $\tra_1, \tra_2$ over $\Sigma$, whether 
$\tra_1\subseteq_\sync \tra_2$ (resp. $\tra_1 \equiv_\sync
\tra_2$). We say that $\tra_1$ is \emph{sequentially $\sync$-uniformisable} if it
admits a sequential uniformiser $U$ such that $U\subseteq_\sync \tra_1$, and in that case $U$ is called a
sequential $\sync$-uniformiser of $\tra_1$ (seq-$\sync$-uniformiser
for short). The \emph{sequential $\sync$-uniformisation
  problem} asks whether a given transducer is
seq-$\sync$-uniformisable. 



It should be clear from the definition that $\mathbb{I}$-inclusion
implies $\sync$-inclusion for any resynchroniser $\sync$, which in
turn implies $\mathbb{U}$-inclusion. As a matter of fact, it is easy
to see that $\mathbb{U}$-inclusion is equivalent to classical
inclusion. The same remarks can be made for equivalence and
sequential uniformisation, and therefore, as a consequence of Theorem~\ref{thm:undecunif}, we get:


% The next proposition states that $\sync$-inclusion and
% $\sync$-equivalence are weaker than $\mathbb{I}$-inclusion and $\mathbb{I}$-equivalence, and
% stronger than $\mathbb{U}$-inclusion and $\mathbb{U}$-equivalence.
% follows from the fact that $\mathbb{I} \subseteq \sync \subseteq
% \mathbb{U}$ for all synchronisers $\sync$.  
  

% \begin{proposition}
    % Given a synchroniser $\sync$ and two transducers $\tra_1,\tra_2$, the
    % following holds:\\
    % \begin{center}
    % \begin{tabular}{ll@{\hspace{5mm}}llllllllllllllll}
        % 1. & if $\tra_1\subseteqq_{\mathbb{I}} \tra_2$, then $\tra_1\subseteqq_\sync \tra_2$, &
                                                                    % 1. & if $\tra_1 \equiv_{\mathbb{I}} \tra_2$, then $\tra_1 \equiv_\sync \tra_2$,\\
        % 2. &  if $\tra_1\subseteqq_\sync \tra_2$, then 
          % $\tra_1\subseteqq_{\mathbb{U}} \tra_2$, & 2. & if $\tra_1 \equiv_\sync \tra_2$, then 
          % $\tra_1 \equiv_{\mathbb{U}} \tra_2$.
    % \end{tabular}
    % \end{center}
% \end{proposition}



% Similarly to the inclusion and equivalence problems, the
% $\sync$-uniformisation is stronger than the
% $\mathbb{I}$-uniformisation, and weaker than the
% $\mathbb{U}$-uniformisation.
% \begin{proposition}
    % Given a synchroniser $\sync$ and a transducer $\tra$, the
    % following holds:\\
    % \begin{center}
    % \begin{tabular}{ll@{\hspace{5mm}}llllllllllllllll}
        % 1. & if $\tra$ is $\mathbb{I}$-uniformisable, then it is $\sync$-uniformisable,\\
        % 2. & if $\tra$ is $\sync$-uniformisable, then it is $\mathbb{U}$-uniformisable.
    % \end{tabular}
    % \end{center}
% \end{proposition}

% A relation may be synchronised by two different languages $L_1$ and
% $L_2$, but the following proposition shows that these two languages
% can then be synchronised by the universal synchroniser $\mathbb{U}$. 

% Different transducers might define the same relation. However, the following
% proposition shows that such transducers can be synchronised by the universal
% synchroniser $\mathbb{U}$.

% \begin{proposition}
    % The following statements are equivalent:
    % \begin{enumerate}
      % \item $\tra_1 \subseteqq \tra_2$ 
      % \item $\tra_1 \subseteqq_{\mathbb{U}} \tra_2$ 
      % \item there
        % exists a synchroniser $\sync$ such that $\tra_1\subseteqq_\sync
        % \tra_2$. 
        % \end{enumerate}
% \end{proposition}


% Consequently, the $\mathbb{U}$-inclusion problem is equivalent
% to the inclusion problem for finite state transducers. Similar results
% hold for the  $\mathbb{U}$-equivalence and $\mathbb{U}$-uniformisation
% problems, yielding the following result.

\begin{theorem}
    The $\mathbb{U}$-inclusion, $\mathbb{U}$-equivalence, sequential
    $\mathbb{U}$-uniformisation problems for rational transductions are undecidable. 
\end{theorem}

%%% transducer Variables:
%%% mode: latex
%%% TeX-master: "decision.tedx"
%%% End:


==> On Equivalence and Uniformisation Problems for Finite Transducers/delay.tex <==
\vspace{.5mm}
\noindent\textbf{Bounded delay resynchronisers}\label{sec:delay} 
The notion of \emph{delay} between outputs of transducers is a
powerful way of comparing transducers, which has been used, for
instance, to characterise sequential functions
\cite{berstel2009}. Intuitively, the delay between two runs on the
same input is a parameter that measures how a run is ahead of the
other, and the lag is the maximal delay over prefixes of the two
runs. We adapt the notion of delay and lag to coloured words and
define delay resynchronisers as resynchronisers that apply a fixed
delay to words in $\inouta^*$ (our notion of lag is not related to the one from \cite{conf/stacs/FigueiraL14}). 
Our results show that delay resynchronisers form
a fundamental class of resynchronisers. 



% Since bounded delay resynchronisers are rational, their associated
% decision problems are decidable. We give complexity bounds for
% uniformisation modulo bounded delay. We also prove that inclusion,
% equivalence and uniformisation modulo bounded delay are not complete,
% in the sense that two transducers may be equivalent but not bounded
% delay equivalent. 


% Intuitively, for any two equivalent words $u,v\in(\inouta)^*$, the
% delay between $u$ and $v$ is a parameter that measure, along 




% A particular and powerful way of comparing how two transducers produce their
% outputs on the same input is via the notion of \emph{delay} between
% outputs. In this section, we study stronger versions of equivalence,
% inclusion and uniformisation problem modulo bounded
% delay. Intuitively, for instance for the equivalence problem, we
% require that the two transducers that are compared produce their
% output in a similar manner, where ``similar'' is formalised here via
% a notion of bounded delay. 


% We first define formally the notion of delay, and show that the
% new decision problems are equivalent to decision problems modulo
% rational synchronisers. In other words, applying a bounded delay to 
% a sequence in $(\inouta)^*$ can be done by a rational synchroniser, and therefore decidability of the
% bounded delay decision problems follows from the
% results of Section \ref{sec:}. However, it turns out that  bounded
% delay synchronisers is an important class of rational synchronisers: for large
% classes of transducers, they provide a complete procedures to test of
% equivalence and inclusion. 




The \emph{delay} between two words $u$ and $v$ over an alphabet
$\Sigma$ is the element
from the free group $G_\Sigma$ defined by $\del(u,v) = u^{-1} v$. 
E.g., $\del(ab,acd) = b^{-1}cd$. Note that $\del(u,v)\in \Sigma^*$ iff
$u\preceq v$, and $\del(u,v)\in (\Sigma^{-1})^*$ iff $v\preceq u$. 
The \emph{lag mapping} $\lag : (\inouta)^* \times (\inouta)^* \rightarrow
\mathbb{N} \cup \{+\infty\}$ gives the maximal length of the delay between the output part of
two words in $(\inouta)^*$ that have the same input. It is the metric defined by
$\lag(u,v)=+\infty$ if $\pi_\inp(u)\neq \pi_\inp(v)$. If $\pi_\inp(u)
= \pi_\inp(v)$, then $u$ and $v$ can be decomposed into 
$u = u_0a_1u_1 \ldots u_{n-1}a_nu_n$ and $v = v_0a_1v_1 \ldots
a_{n-1}b_nv_n$, such that $a_1, \ldots, a_n \in \ina$, $u_0,v_0,
\ldots, u_n,v_n \in (\outa)^*$. Then $\lag(u,v) = \max_{0 \leq i \leq
  n} |\del(u_0 \ldots u_i,v_0 \ldots v_i)|$. %
% Note that if $\lag(u,v)<+\infty$, then $u$ and $v$ are equivalent, and
% therefore for all $0\leq i\leq n$, $\del(u_0 \ldots u_i,v_0 \ldots v_i)\in\Sigma^*\cup
% (\Sigma^{-1})^*$. 
As an example, for $n\geq 1$, take $u_n = a^\inp a^\outp (a^\inp)^n$ and $v_n =
(a^\inp)^n a^\inp a^\outp$. Then for all $n\geq 1$, $\lag(u_n,v_n){=}
1$. Note that the occurrence of $a^\outp$ in $u_n$ is arbitrary
far from that of $a^\outp$ in $v_n$. 

We now define the $k$-delay resynchroniser
$\mathbb{D}_k$. Intuitively, it can shift output symbols of a word $u$
to the left or to the right, as long as the lag between $u$ and the
new word obtained this way is bounded by $k$. Formally, the
\emph{$k$-delay resynchroniser} is defined by $\dsync_k\ =\ \{
(u,v)\in (\inouta)^2\mid u\sim_{\inout}v\wedge \lag(u,v)\leq
k\}$. We define the $k$-inclusion, $k$-equivalence and
sequential $k$-uniformisation problems as the corresponding $\dsync_k$-decision
problems, and write $\subseteq_k$ and $\equiv_k$ instead of 
$\subseteq_{\dsync_k}$ and $\equiv_{\dsync_k}$
respectively. We also say that a transduction is seq-$k$-uniformisable
if it is seq-$\dsync_k$-uniformisable. An important property of $\dsync_k$ is:
\begin{restatable}{proposition}{dsyncrational}\label{prop:dsynckrat}
    For all $k\geq 0$, $\dsync_k$ is rational. 
\end{restatable}
As a direct consequence of the latter proposition and
Theorem~\ref{thm:rat}, the $k$-delay decision problems are all
decidable. We can be more precise:
\begin{restatable}{theorem}{decisionkdelay}
    For all $k\geq 0$, the $k$-inclusion, $k$-equivalence
    and sequential $k$-uniformisation problems are decidable and
    \textsc{ExpSpace-hard} if $k$ is part of the input. If $k$ is
    fixed, then the $k$-inclusion and $k$-equivalence problems are
    \textsc{PSpace-complete}, and the sequential $k$-uniformisation problem is
    \textsc{ExpTime-complete}.
\end{restatable}



% \paragraph{Bounded delay problems for transducers} 
% Given $k \in \mathbb{N}$ and two transducers $\tra_1$ and $\tra_2$, we
% say that $\tra_1$ is $k$-delay included in $\tra_2$, denoted by
% $\tra_1 \subseteq_k \tra_2$, if for every word $w \in \lang{\tra_1}$
% there exists a word $w' \in \lang{\tra_2}$ such that $w$ and $w'$ are
% equivalent, and $\lag(w,w') \leq
% k$. Similarly,  $\tra_1$ and $\tra_2$ are $k$-delay equivalent, denoted by
% $\tra_1 \equiv_k \tra_2$, if $\tra_1 \subseteq_k \tra_2$ and $\tra_2
% \subseteq_k \tra_1$. Finally, we say that $\tra_1$ is $k$-delay uniformisable if it admits a uniformiser $\uni$ such that $\uni \subseteq_k \tra_1$.
% With $k$ being part of the input, we can naturally define the
% $k$-delay inclusion, equivalence and uniformisation problems. 


% We first show that $k$-delay inclusion, equivalence and uniformisation
% are equivalent to inclusion, equivalence and uniformisation modulo
% rational synchronisers. 


% \begin{proposition}\label{prop:equivsynchro}
% Let $k \in \mathbb{N}$, and let $\tra_1,\tra_2,\tra$ be transducers. There exists a rational synchroniser $\dsync_k$
% such that 
% \begin{itemize}
    % \item $\tra_1$ and $\tra_2$ are $k$-delay equivalent iff $\tra_1$
      % and $\tra_2$ are equivalent modulo $\dsync_k$,
    % \item $\tra_1$ is $k$-delay included in $\tra_2$ iff $\tra_1$ is
      % included in $\tra_2$ modulo $\dsync_k$,
    % \item $\tra$ is $k$-delay uniformisable iff $\tra$ is
      % uniformisable modulo $\dsync_k$. 
% \end{itemize}
% Moreover, $\dsync_k$ can be defined by a transducer with $O(|\Sigma|^k)$
% states. 
% \end{proposition}





Even if inclusion is undecidable while $k$-inclusion is decidable, it
could be the case that inclusion reduces to $k$-inclusion, for
some $k$ that cannot be computed. We show that that it is not the
case, by using the transducers of Fig.~\ref{fig:notk}. 


% : there are transducers $\tra_1,\tra_2$ such that $\tra_1\subseteq
% \tra_2$ but $\tra_1\not\subseteq_k\tra_2$ for any $k$. We prove
% similar results for equivalence and uniformisation. In the following
% proposition, $\subseteq_k$ and $\equiv_k$ are seen as binary relations
% % on transducers over a fixed unary alphabet $\Sigma$, and we denote by $\text{Unif}_k$ the class of transducers that are $k$-delay
% uniformisable, and by $\text{Unif}$ the class of transducers that are
% uniformisable.

\begin{restatable}{proposition}{propapprox}\label{prop:notcomplete}
    There exist transducers $\tra_1,\tra_2,\tra$ such that
    $\tra_1\equiv \tra_2$, $\tra_1\subseteq \tra_2$ and $\tra$ is
    seq-uniformisable, but for all $k\geq 0$,
    $\tra_1\not\equiv_k\tra_2$, $\tra_1\not\subseteq_k\tra_2$, and $\tra$ is not seq-$k$-uniformisable.
    % $(\bigcup_{k=0}^{+\infty} \subseteq_k)\ \subsetneq\ (\subseteq)$, 
    % $(\bigcup_{k=0}^{+\infty} \equiv_k)\ \subsetneq\ (\equiv)$,
    % $(\bigcup_{k=0}^{+\infty}\text{Unif}_k)\ \subsetneq\ \text{Unif}$.     
\end{restatable}

\begin{proof}
    Consider $\tra_1,\tra_2$ of Fig.\ref{fig:notk} and pairs of the
    form $(a^{n+1},a^{2n})\in\rel{\tra_1}=\rel{\tra_2}$. They both
    accept these pairs but $\tra_2$ will be arbitrarily late compared
    to $\tra_1$.  Consider now the transducer $T$ and its sequential uniformiser
    $U$. On inputs $a^nB$, $U$ will be arbitrarily ahead of $T$, and
    one can show that is the case for \emph{any} seq-uniformiser of $T$.
\end{proof}





Finally, we show that for real-time transductions, $k$-delay resynchronisers subsume any rational
resynchroniser $\sync$, in the sense that $\sync$-inclusion implies 
$k$-inclusion, for some $k$ that depends on $\sync$. Similar
results hold for equivalence and sequential uniformisation. The idea is that a
rational synchroniser cannot advance or delay the production of
outputs arbitrarily far away with a finite set of states. 

\begin{restatable}{theorem}{thmsyncdel}\label{thm:thmsyncdel}
    Let $\sync$ be a rational synchroniser (given by a transducer). 
    Let $\tra_1,\tra_2,\tra$ be real-time transducers. 
    There exists a computable integer $k\in\mathbb{N}$ such that:
   $(i)$ if $\tra_1\subseteq_\sync \tra_2$, then
        $\tra_1\subseteq_k \tra_2$, $(ii)$  if $\tra_1\equiv_\sync \tra_2$, then
        $\tra_1\equiv_k \tra_2$, and $(iii)$ if $\tra$ is seq-$\sync$-uniformisable, then $\tra$ is
        seq-$k$-uniformisable.
\end{restatable}

\noindent One cannot drop the real-time assumption in the latter
theorem. Indeed consider the following transducers
$\tra_1,\tra_2,\sync$, for which $\tra_1{\equiv_\sync} \tra_2$ but
$\tra_1, \tra_2$ are not $k$-equivalent for any $k$:
\vspace{-1mm}
\begin{center}
\begin{tikzpicture}[->,>=stealth',auto,node
    distance=1cm,thick,scale=0.7,every node/.style={scale=0.7}]
  \tikzstyle{every state}=[fill=yellow!30,text=black]
  % \tikzstyle{every edge}=[draw=black,text=red]
  \tikzstyle{initial}=[initial by arrow, initial where=left, initial text=]
  \tikzstyle{accepting}=[accepting by arrow, accepting where=right, accepting text=]
  \tikzstyle{acceptingdown}=[accepting by arrow, accepting where=below, accepting text=]

  \tikzstyle{initialT1}=[initial by arrow, initial where=left, initial
  text={$\tra_1\ :\ $}]
  \tikzstyle{initialT2}=[initial by arrow, initial where=left, initial
  text=$\tra_2\ :\ $]
  \tikzstyle{initialS}=[initial by arrow, initial where=left, initial
  text=$\sync\ :\ $]

  \node[initialT1,state] (A) at(0,0) {};
  \node[accepting,state] at(2,0) (B)  {};
  \path (A) edge node {\trans{a}{\epsilon}} (B);
  \path (B) edge [loop above] node {\trans{\epsilon}{b}} (B);

  \node[initialT2,state] (C) at(6,0) {};
  \node[accepting,state] at(8,0) (D)  {};
  \path (C) edge node {\trans{a}{\epsilon}} (D);
  \path (C) edge [loop above] node {\trans{\epsilon}{b}} (C);

  \node[initialS,state] (E) at(12,0) {};
  \node[state] at(14,0) (F)  {};
  \node[accepting,state] at(16,0) (G)  {};
  \path (E) edge node {\trans{a^\inp}{\epsilon}} (F);
  \path (F) edge [loop above] node {\trans{b^\outp}{b^\outp}} (F);
  \path (F) edge node {\trans{\epsilon}{a^\inp}} (G);
\end{tikzpicture}
\end{center}
\vspace{-1mm}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> On Equivalence and Uniformisation Problems for Finite Transducers/drat-uniformizer-to-strategy.tex <==
\newcommand{\pump}[2]{\mathit{pump}_{#1}(#2)}
\newcommand{\Pump}[2]{\mathit{Pump}_{\ge #1}(#2)}

We prove the existence of a winning strategy for Output in case that $R_\tra$
is uniformized by a sequential transducer. A note for the reader who
is not very familiar with this kind of game-theoretic reasoning: The
strategy that we construct below is not positional, it uses a memory of unbounded size. Furthermore, we do not even need to care whether we can compute the individual moves. Proving the existence of some strategy is sufficient and implies the existence of a positional strategy, as assumed in the proof of Lemma~\ref{lem:drat-strategy-to-uniformizer}.

\begin{lemma}\label{lem:drat-uniformizer-to-strategy}
  If $R_\tra$
  can be uniformized by a sequential transducer, then Output has a
  winning strategy in $\game_\tra$.
\end{lemma}



The rest of this section is devoted to the proof of Lemma~\ref{lem:drat-uniformizer-to-strategy}, which requires some definitions and other lemmas. For the construction of the strategy, we split the transformation sequence in a game position in two parts, both of length at most $K$. So we consider game positions of the form $(p,\rho\xi,d)$ with $|\rho| \le K+1$ and $|\xi| \le K$. The moves of type (Out3), which apply the operation $\reduce{\cdot}$ to an infix of the transformation sequence, are only applied to the second part $\xi$ of the transformation sequence. The first part $\rho$ remains fixed until it is consumed by an output move of type (Out2). 

Input word $u$ that generates the part $\xi$ of the transformation sequence is stored in the memory of the strategy, together with the information to which parts the operation $\reduce{\cdot}$ was applied (the operation $\reduce{\cdot}$ is applied to parts of the transformation sequence, but each such part corresponds to a part of $u$).
This leads to a structure of the form $(u,M)$ with a set $M$ of edges $(i,j)$, where $i < j$ are positions in $u$. These edges are well-nested (they do not cross). In the construction of the strategy, we need to refer to words that are obtained from $u$ by pumping the parts of $u$ enclosed by an edge.  Hence, we refer to $(u,M)$ as a \emph{pump-word}. 

Formally, pump-words $(u,M)$ and their corresponding transformation sequences $\rho_{(u,M)}$ are defined inductively as detailed below. 
Along the inductive definition we also define how to concatenate two pump-words.

%For these pumping operations we require that the edges $(i,j)$ are such that the infix $u[i,j]$ of $u$, and the infix of $\xi$ corresponding to $u[i,j]$ are idempotent and absorbed. This ensures that pumping the infixes corresponding to the edges does not change the profile of the word.
%
%Before we give the precise conditions that pump-words $(u,M)$ have to satisfy, we  define 

\begin{definition}\label{def:pump-word}
\begin{enumerate}
\item For each $u \in \Sigmaend^*$, $(u,\emptyset)$ is a pump-word. The transformation sequence of $(u,\emptyset)$ is $\rho_{(u,\emptyset)} := \rho_u$, the transformation sequence induced by $u$.
\item The concatenation of two pump-words $(u_1,M_1)$ and $(u_2,M_2)$ is defined in the expected way as $(u_1,M_1)(u_2,M_2) = (u_1u_2,M_1 \cup (M_2 + |u_1|))$, where $M_2 + |u_1|$ denotes the set of edges in $M_2$ shifted by $|u_1|$ to the right. For example $(aba,\{(1,2)\})(bbc,\{(1,3)\}) = (ababbc,\{(1,2),(4,6)\}$. 

%If $(u,M) = (u_1,M_1)(u_2,M_2)$, then the transformaiton sequence is defined as $\rho_{(u,M)} = \rho_{(u_1,M_1)} \circ  \rho_{(u_2,M_2)}$.

\item Let $(u,M)$ be a pump-word and let $\xi = \rho_{(u,M)}$ to simplify notation. Let $\xi = \xi_1\xi_2\xi_3$, where $\xi_1,\xi_2,\xi_3$ are transformation sequences and $|\xi_2| \ge 2$. Let $(u,M) = (u_1,M_1)(u_2,M_2)(u_3,M_3)$ be the corresponding split of $(u,M)$, that is, $\rho_{(u_i,M_i)} = \xi_i$ for all $i \in \{1,2,3\}$. 
If $P_{x_2}$ is idempotent and $P_{u_2}$ is idempotent, then $(u,M') = (u_1,M_1)(u_2,M_2 \cup \{(1,|u_2|)\})(u_3,M_3)$ is a pump-word, and $\rho_{(u,M')} := \xi_1\reduce{\xi_2}\xi_3$ is the transformation sequence of $(u,M')$.

Note that $M' = M \cup \{(|u_1|+1,|u_1|+|u_2|)\})$ according to the definition of concatenation of pump-words. \qed
\end{enumerate}
\end{definition}
In point~3 of Definition~\ref{def:pump-word}, we implicitly assume that the split $(u,M)) = (u_1,M_1)(u_2,M_2)(u_3,M_3)$ that is induced by the split $\xi = \xi_1\xi_2\xi_3$ does not ``cut'' any edge of $M$ (all edges of $u$ are inside $u_1$, $u_2$, or $u_3$). This follows from the fact that an infix $v$ of $u$ that is enclosed by an edge only contributes a single transformation $\reduce{\rho_v}$ to  $\rho_{(u,M)}$.

%Point 2 is only needed to define the concatenation of pump-words, which is used in point 3. 

As mentioned earlier, the edges in a pump-word mark factors that we want to pump. In the following, when we speak of a pumping factor, then we refer to an infix of $u$ that corresponds to an edge. For a pump-word $(u,M)$ and a number $k$, we define the set $\Pump{k}{(u,M)}$, which is obtained by repeating each pumping factor at least $k$ times:

\begin{itemize}
\item If $M = \emptyset$, then $\Pump{k}{(u,M)} = \{u\}$.
%\item If $(u,M) = (u_1,M_1)(u_2,M_2)$, then $\pump{k}{(u,M)} = \pump{k}{(u_1,M_1)}\pump{k}{(u_2,M_2)}$ and $\Pump{k}{(u,M)} = \Pump{k}{(u_1,M_1)}\Pump{k}{(u_2,M_2)}$.
\item If $(u,M) = (u_1,M_1)(u_2,M_2 \cup \{(1,|u_2|)\})(u_3,M_3)$ as in point 3 of Definition~\ref{def:pump-word}, then
 $\Pump{k}{(u,M)} = \bigcup_{\ell \ge k} \Pump{k}{(u_1,M_1)}(\Pump{k}{(u_2,M_2)})^\ell\Pump{k}{(u_3,M_3)}$ 
\end{itemize}
Clearly, $\Pump{k}{(u,M)}$ is a regular set for each $k$ and each $(u,M)$.

The condition on the profiles of pumping factors being idempotent, ensures that pumpings do not change profiles, as expressed in the following lemma.
\begin{lemma} \label{lem:pump-word-profile}
If $(u,M)$ is a pump-word, then $P_w = P_u$ for each word $w \in \Pump{1}{(u,M)}$.  
\end{lemma}
\begin{proof}
  The proof is by induction on the complexity of $(u,M)$, which is a mapping $\varphi: \nat \rightarrow \nat$ where $\varphi(n)$ is the number of edges in $M$ that are of nesting depth $n$. The nesting depth of an edge $(i,j)$ is defined as $1$ if there are no other edges inside $(i,j)$, and otherwise it is $n+1$ if the maximal nesting depth of an edge inside $(i,j)$ is $n$.
Note that $\varphi(n) > 0$ for only finitely many $n$.

We use the a lexicographic ordering for comparing these mappings, letting $\varphi_1 < \varphi_2$ if $\varphi_1(n) < \varphi_2(n)$ for the biggest $n$ with $\varphi_1(n) \not= \varphi_2(n)$ (note that such an $n$ exists if $\varphi_1 \not= \varphi_2$, as there are only finitely many non-zero entries). This is a well-ordering \cite{Dickson13} and thus can be used for an induction.

For the induction base, if $\varphi$ maps everything to $0$, then $M = \emptyset$ and $w = u$. 

So consider the last edge that has been added to $M$ according to Definition~\ref{def:pump-word}. This means that $(u,M) = (u_1,M_1)(u_2,M_2 \cup \{1,|u_2|\})(u_3,M_3)$, where the edge enclosing $u_2$ is the last one that was added. Then $w = w_1w_{2,1}\cdots w_{2,\ell}w_3$ with $w_1 \in \Pump{k}{(u_1,M_1)}$, $w_{2,1},\cdots, w_{2,\ell} \in \Pump{k}{(u_2,M_2)}$, and $w_3 \in \Pump{k}{(u_3,M_3)}$. Note that $(u_1,M_1)(u_2,M_2)^\ell(u_3,M_3)$ is a pump-word, and its complexity is smaller than the one of $(u,M)$ because the edge enclosing $u_2$ is removed and the iteration of $(u_2,M_2)$ only increases the number of edges of smaller nesting depth.

Then by induction, $P_{w_1w_{2,1}\cdots w_{2,\ell}w_3} = P_{u_1(u_2)^\ell u_3}$, and since $P_{u_2}$ is idempotent, we obtain $P_{u_1(u_2)^\ell u_3} = P_{u_1u_2u_3} = P_u$ for $\ell \ge 1$.
\end{proof}


The pump-words that we build during the strategy construction apply point 3 of Definition~\ref{def:pump-word} to saturation witnesses (see Section~\ref{subsec:profiles-and-saturated-sequences}). So they satisfy some further properties that, intuitively, ensure that outputs matching pumped words can be replaced by outputs matching the unpumped words. We refer to such pump-words as \emph{safe}:
 
\begin{definition}\label{def:safe-pump-word}
A pump-word is called \emph{safe} if in Definition~\ref{def:pump-word}(3) the following additional conditions are satisfied (using the same notations as in Definition~\ref{def:pump-word}(3)): 
\begin{itemize}
\item $M_3 = \emptyset$, so there are no edges after the one that is newly introduced.
\item $P_{\xi_1} = P_{\xi_1}P_{\xi_2}$ ($\xi_2$ is absorbed by $\xi_1$).
\item $P_{u_1} = P_{u_1}P_{u_2}$ ($u_2$ is absorbed by $u_1$).
\end{itemize}
The connection of saturation witnesses (see Section~\ref{subsec:profiles-and-saturated-sequences}) and the condition for safe pump-words is as follows. Let $\xi = \tau_1 \cdots \tau_{|\xi|}$, and  let $(u,M) = (u_1',M_1') \cdots (u_{|\xi|}',M_{|\xi|}')$ be the corresponding split of $(u,M)$ (that is, $\rho_{(u_i',M_i')} = \tau_i$). Let $\bar{P} = P_{u_1},\cdots, P_{u_{|\xi|}}$. Then the conditions for safe pump-words implies that $\xi_1\xi_2\xi_3$ is a saturation witness for $\xi$ and $\bar{P}$. Since $(u,M)$ determines $\xi = \rho_{(u,M)}$, and $\bar{P}$, we call this a \emph{saturation witness for $(u,M)$}. \qed
\end{definition}
The reason for considering pump-words and safe pump-words (and not just defining the latter) is that in a decomposition of a safe pump-word $(u,M) = (u_1,M_1)(u_2,M_2)(u_3,M_3)$, the part $(u_2,M_2)$ needs not to be safe (the condition of safe pump-word refers to the prefixes before the pumping factors). However, $(u_2,M_2)$ is a pump-word because being idempotent is a local property that does not depend on the prefix. 


The following lemma is essential for the strategy construction. It basically states that if an output word that matches a large pumping of $(u,M)$, then there is also an output word matching $\rho_{(u,M)}$, that is, an output that is consumed outside the pumping factors of $(u,M)$.
\begin{lemma} \label{lem:output-large-pumping}
  Let $(u,M)$ be a safe pump-word, $p,q \in Q$, and $v \in \Sigmaend^*$ be an output word such that there is $w \in \Pump{3|v|}{(u,M)}$ with $v \in \Lout(p,\rho_w,q)$. Then $\Lout(p,\rho_{(u,M)},q) \not= \emptyset$.
\end{lemma}
\begin{proof}
  The proof is by induction on the complexity of $(u,M)$, as in the proof of Lemma~\ref{lem:pump-word-profile}. If $M = \emptyset$, and the claim obviously holds because $w = u$ (there are no pumping factors) and $\rho_u = \rho_{(u,\emptyset)}$.

So consider the last edge that has been added to $M$ according to Definition~\ref{def:safe-pump-word}. This means that $(u,M) = (u_1,M_1)(u_2,M_2 \cup \{1,|u_2|\})(u_3,M_3)$, where the edge enclosing $u_2$ is the last one that was added. And as in the definition of pump-words, let $\xi_i = \rho_{(u_i,M_i)}$. We want to show that $\Lout(p,\xi_1\reduce{\xi_2}\xi_3,q) \not = \emptyset$.

By definition of $\Pump{3|v|}{(u,M)}$, we can write $w = w_1 w_{2,1}\cdots w_{2,\ell} w_3$ with $\ell \ge 3|v|$, $w_1 \in \Pump{3|v|}{(u_1,M_1)}$, $w_3 \in \Pump{3|v|}{(u_3,M_3)}$, and $w_{2,i} \in \Pump{3|v|}{(u_2,M_2)}$. Note that $P_{w_1} = P_{u_1}$, $P_{w_{2,i}} = P_{u_2}$, and $P_{w_3} = P_{u_3}$ by Lemma~\ref{lem:pump-word-profile}.

According to the definition of $\Lout(p,\rho_w,q)$, we can write $v = v_1v_{2,1}\cdots  v_{2,\ell} v_3$ with $v_1 \in \Lout(p,\rho_{w_1},q_2^0)$, each $v_{2,i} \in \Lout(q_2^{i-1},\rho_{w_{2,i}},q_2^i)$, and $v_3 \in \Lout(q_2^\ell,\rho_{w_3},q)$ for some states $q_2^0, \ldots, q_2^\ell$.

Since $\ell \ge 3|v|$, there must be an $i < 2|v|$ with $v_{2,i} = v_{2,{i+1}} = \varepsilon$. By definition of profiles we obtain $(q_2^{i-1},\varepsilon, q_2^i) \in P_{u_2}$ and $(q_2^i,\varepsilon, q_2^{i+1}) \in P_{u_2}$.  Since $P_{u_2}$ is idempotent by definition of pump-words, we obtain $(q_2^{i-1},\varepsilon, q_2^{i+1}) \in P_{u_2}$, and thus $q_2^i = q_2^{i+1}$ (see Lemma~\ref{lem:profile-properties}). We conclude that $(q_2^i, \varepsilon, q_2^i) \in P_{u_2}$, and $q_2^j = q_2^i$ and $v_{2,j} = \varepsilon$ for each $i \le j \le \ell$. 

Let $q_2 := q_2^i$, $w' =  w_1w_{2,1} \cdots w_{2,{2|v|}}$ and $v' = v_1v_{2,1} \cdots v_{2,{2|v|}}$. As a consequence of the above considerations, $v' \in \Lout(p,\rho_{w'},q_2)$.
Note that $(u_1,M_1)(u_2,M_2)^{2|v|}$ is a safe pump-word of smaller complexity than the one of $(u,M)$ (the edge enclosing $u_2$ in $(u,M)$ was removed, and the iteration of $(u_2,M_2)$ only adds edges of smaller nesting depth). Furthermore $w' \in \Pump{3|v|}{(u_1,M_1)(u_2,M_2)^{2|v|}}$, and $3|v| \ge 3|v'|$. We can thus apply the induction and obtain that $\Lout(p,\xi_1(\xi_2)^{2|v|},q_2) \not= \emptyset$. Since  $P_{\xi_2} = P_{\xi_2}P_{\xi_2}$ and $P_{\xi_1} = P_{\xi_1}P_{\xi_2}$, we conclude that $\Lout(p,\xi_1,q_2) \not= \emptyset$. 

From $(q_2,\varepsilon,q_2) \in P_{u_2}$ (as deduced above), we obtain $\varepsilon \in \Lout(q_2,\rho_{u_2},q_2)$, which implies $\varepsilon \in \Lout(q_2,\reduce{\rho_{u_2}},q_2)$ (see Lemma~\ref{lem:empty-word-traversal}). Since $\reduce{\rho_{u_2}} = \reduce{\rho_{(u_2,M_2)}} = \reduce{\xi_2}$, we conclude that $\Lout(q_2,\reduce{\xi_2},q_2) \not= \emptyset$.

Finally, note that $M_3 = \emptyset$ in the definition of safe pump-word. Hence $w_3 = u_3$, and $\xi_3 = \rho_{u_3}$. Thus $v_3 \in \Lout(q_2^\ell,\xi_3,q)$ because $P_{w_3} = P_{u_3}$.

Putting all these together, we obtain that $\emptyset \not= \Lout(p,\xi_1,q_2)\Lout(q_2,\reduce{\xi_2},q_2)\Lout(q_2,\xi_3,q) \subseteq \Lout(p,\xi_1\reduce{\xi_2}\xi_3)$ as desired. 
\end{proof}


\subsubsection*{An invariant for the strategy}

Before we start the construction of the strategy, we introduce one more terminology concerning uniformizers that  simplifies the presentation below. Recall the definition of the relation $R_p^\rho$ from Section~\ref{subsec:langauges-and-relations-of-transformation-sequences}. Every output in this relation has to start with a prefix in $\Lout(p,\rho)$. We say that a sequential uniformizer $S$ of $R_p^\rho$ is a \emph{$(p,\rho)$-uniformizer} if 
\begin{itemize}
\item in every run, the first non-empty output that $S$ produces has a prefix in $\Lout(p,\rho)$, and
\item $S$ outputs the endmarker only if it reads the endmarker on the input.
\end{itemize}
So with $(p,\rho)$-uniformizers we exclude the case that the prefix from $\Lout(p,\rho)$ is built up incrementally along several transitions, and the case that an endmarker is produced on the output before the endmarker has appeared on the input. It is quite easy to see that working with $(p,\rho)$-uniformizers is not a restriction.

\begin{remark}
If there is a sequential uniformizer for $R_p^\rho$, then there is also a $(p,\rho)$-uniformizer. 
\end{remark}
\begin{proof}
First note that for each $q \in Q$ the language $\Lout(p,\rho,q)$ is regular. 
Given a sequential uniformizer $S$ for $R_p^\rho$, one can construct a $(p,\rho)$-uniformizer $S'$ as follows. It mimics the transitions of $S$ but instead of producing output, it simulates 
DFAs for each $\Lout(p,\rho,q)$ on the output that $S$ would have produced. If the DFA for $\Lout(p,\rho,q)$ reaches an accepting state, then $S'$ produces some output word in $\Lout(p,\rho,q)$, appending the possibly remaining part $v$ of the output from the last transition. 

The property concerning the endmarker is easily achieved by delaying the output of it to the transition that reads $\dashv$ on the input.
\end{proof}

%A memory state of the strategy $f_\tra$ that we construct from $\tra$ is of the form $[(d,p,\rho,\xi),(u,M)]$ where  $(d,p,\rho\xi)$ is the current vertex of the play, $|\rho|,|\xi|\le K$, and $(u,M)$ is a pump-word with $\rho_{(u,M)} = \xi$. 
We construct a strategy $f_\tra$ from $\tra$, such that an invariant is maintained in each move, from which follows that $f_T$ is winning. The invariant is stated below. Condition (Inv0) only describes some properties on the structure of the memory that is used for $f_\tra$. Condition (Inv1) implies that $f_\tra$ is a winning strategy. The conditions (Inv2) and (Inv3) state intuitively that it is still possible to uniformize the remaining relation w.r.t.\ the input and output moves that have already been played.

For a sequential transducer $S$ and an input word $w$, we write $S(w)=v$ if $S$ produces output $v$ when reading input $w$.

\begin{itemize}
\item[(Inv0)] The memory states of $f_\tra$ are of the form $[(p,\rho,d',\xi,d),(u,M)]$, where 
  \begin{enumerate}[(i)]
  \item the current game position is of the form $(p,\rho\xi,d)$ or $(p,\rho\xi,d,a)$ (the memory maintains two parts of the transformation sequence in the game position;  $f_\tra$ only applies moves of type (Out3) to the second part $\xi$);
  \item  $|\rho| \le K+1$, $|\xi| \le K$;
  \item $(u,M)$ is a safe pump-word with $\rho_{(u,M)} = \xi$ ($u$ is the input sequence that induced $\xi$, and $M$ corresponds to the applications of moves of type (Out3));
  \item if $\xi$ is saturated, then a saturation witness for $(u,M)$ is of the form $\xi_1\xi_2\xi_3$ with $\xi_3 = \varepsilon$ (new edges to $u$ will be added only at the end of the word);
  \item $A_\dom: d' \xrightarrow{u} d$ (before reading $u$, the automaton $A_\dom$ was in state $d'$). 
  \end{enumerate}
\item[(Inv1)] If $d \in F_\dom$, then $\rho = \xi = \varepsilon$ and $p \in F$.
\item[(Inv2)] If $d \notin F_\dom$, then there is a $(p,\rho)$-uniformizer, and the domain of $R_p^{\rho}$ contains all words from $L(A_\dom,d')$, which is the set of word accepted by  $A_\dom$ from state $d'$. 
\item[(Inv3)] For every $(p,\rho)$-uniformizer $S$ there is $w \in \Pump{|S|!}{(u,M)}$ such that $S(w) = \varepsilon$.
\end{itemize}

The last condition (Inv3) is used to build a $(q,\xi)$-uniformizer (ensuring (Inv2) in the new vertex), once the strategy is ready to play an output in $\Lout(p,\rho,q)$ that consumes $\rho$ from the lookahead. The choice of $|S|!$ for the number repetitions in the pumping ensures that $S$ enters a loop on each of the pumped factors. This is useful in the proofs below. 


\begin{lemma} \label{lem:invariant-implies-winning}
  If the strategy $f_\tra$ satisfies the properties (Inv0)--(Inv3), then it is a winning strategy. 
\end{lemma}
\begin{proof}
This is a direct consequence of  (Inv1).
\end{proof}


The next lemma is the key lemma for preserving the invariant in a move that produces output. It covers the case that (Inv3) fails after appending the next input letter $a$. Then the goal is to produce output that consumes $\rho$ and to transfer the property (Inv2) to $\xi \circ \tau_a$.
\begin{lemma} \label{lem:propagate-invariant}
Let $[(p,\rho,d',\xi,d),(u,M)]$ be a memory state that satisfies (Inv0)--(Inv3). Let $a \in \Sigmaend$ be such that $S(wa) \not= \varepsilon$ for all $w \in \Pump{|S|!}{(u,M)}$ for some $(p,\rho)$-uniformizer $S$. Then there exists $q \in Q$ such that 
\begin{itemize}
\item $\Lout(p,\rho,q) \not= \emptyset$, 
\item The domain of $R_q^{\xi \circ \tau_a}$ contains all words in $L(A_\dom,d_a)$ with $d_a = \delta_\dom(d,a)$, 
\item and if $a \not= \dashv$, there is a $(q,\xi \circ \tau_a)$-uniformizer.  
\end{itemize}
\end{lemma}
\begin{proof}
By (Inv3), there is  $w \in \Pump{|S|!}{(u,M)}$ such that $S(w) = \varepsilon$. Let $s_0$ be the initial sate of $S$, and $s',s$ be the states of $S$ such that $S: s_0 \xrightarrow{w/\varepsilon} s' \xrightarrow{a/yz} s$, where $y \in \Lout(p,\rho,q)$ for some state $q$ (the first non-empty output contains a prefix in $\Lout(p,\rho)$). This proves the existence of $q \in Q$ such that $\Lout(p,\rho,q) \not= \emptyset$.

Since $S$ does not see the difference between a factor repeated $\ell \ge |S|!$ times or $\ell + k|S|!$ times, one can even find $w_k \in  \Pump{k|S|!}{(u,M)}$ for each $k\ge 1$ such that $S(w_k) = \varepsilon$ and furthermore, $S$ reaches the same state $s'$ after reading $w_k$ for all $k$. So $S: s_0 \xrightarrow{w_k/\varepsilon} s' \xrightarrow{a/yz} s$ for all $k$ 

Let $x \in L(A_\dom,d_a)$. Then $uax \in L(A_\dom,d')$ because:
\[
  A_\dom: d' \xrightarrow{u} d \xrightarrow{a} d_a \xrightarrow{x} F_\dom.
\]
Since the pumped words of $(u,M)$ induce the same state transformation on $A_\dom$ as $u$, we obtain that $w_kax \in L(A_\dom,d')$ for all $k$.
Let $z_x$ be the output produced by $S$ on input $x$ from state $s$. Then
\[
S: s_0 \xrightarrow{w_k/\varepsilon} s' \xrightarrow{a/yz} s \xrightarrow{x/z_x} F_S
\]
for each $k$, where $F_S$ is the set of final states of $S$.
This implies that $\delta^*(q,w_kax,zz_x) = (r_k,\varepsilon,\varepsilon)$ with $r_k \in F$ for each $k$ because $S$ is a $(p,\rho)$-uniformizer. So for each $k$, $zz_x$ has a prefix $v_k$ such that $\delta^*(q,w_ka,v_k) = \delta^*(q_k',a,\varepsilon) = (q_k,\varepsilon,\varepsilon)$ for some state $q_k$. In other words, $v_k \in \Lout(q,\rho_{w_ka},q_k)$.

Since there are only finitely many possible prefixes $v_k$ and states $q_k$,  there are infinitely many $k$ with the same $v_k$ and the same $q_k$. By choosing the corresponding subsequence of $w_1,w_2,\ldots$, we can assume that all $v_k$ and $q_k$ are the same, so we just denote them by $v_1$ and $q_1$.

We obtain that $v_1 \in \Lout(q,\rho_{w_ka},q_1)$ for all $k$. By choosing $k = 3|v_1|$, we can apply Lemma~\ref{lem:output-large-pumping}, and obtain that $\Lout(q,\xi \circ \tau_a,q_1) \not= \emptyset$. 

We can conclude that  $x \in \dom(R_q^{\xi \circ \tau_a})$ as follows. The output word $zz_x$ was shown to be the form $v_1v'$. We can replace the prefix $v_1$ by some word $v'' \in \Lout(q,\xi \circ \tau_a,q_1)$. Then $(x,v''v') \in R_q^{\xi \circ \tau_a}$.

It remains to prove that there is a $(q,\xi \circ \tau_a)$-uniformizer $S'$ in case $a \not= \dashv$. The reason for excluding $\dashv$ is that in this case there are no further transitions of $S$ from $s$.

We already proved that for each input $x \in L(A_\dom,d_a)$, the output word $zz_x$ (as above) is of the form $v_1v'$ with $v_1 \in \Lout(q,\rho_{w'a},q_1)$ for some $w' \in  \Pump{|S|!}{(u,M)}$ with $S:s_0 \xrightarrow{w'/\varepsilon} s'$, and some state $q_1$, such that $\Lout(q,\xi \circ \tau_a,q_1) \not= \emptyset$. And then $(x,v''v') \in R_q^{\xi \circ \tau_a}$ for $v'' \in \Lout(q,\xi \circ \tau_a,q_1)$.

The idea for constructing a $(q,\xi \circ \tau_a)$-uniformizer $S'$ is that we modify $S$ to detect a prefix of the output with the properties of $v_1$ as above, and then replace it by $v''$. To implement this operation, we show that the set of output strings $v_1$ with the above property is regular, by using the following observations:
\begin{itemize}
\item $L_1 := \Pump{|S|!}{(u,M)}$ is regular.
\item $L_2 := \{w' \in \Sigmaend^* \mid S:s_0 \xrightarrow{w'/\varepsilon} s'\}$ is regular.
\item For each $q_1$, the set $L_{q_1}$ of output strings $v_1$ such that there exists $w' \in L_1 \cap L_2$ and $v_1 \in \Lout(q,\rho_{w'a},q_1)$ is regular. An automaton for this set reads $v_1$, guesses $w'$, simulates $\tra$ from $q$ on the pair $(w',v_1)$, and simulates an automaton for $L_1 \cap L_2$ on the guessed $w'$. 
\end{itemize}
So the $(q,\xi \circ \tau_a)$-uniformizer $S'$ simulates  the transitions of $S$ starting from state $s$, and in parallel simulates for each $q_1 \in Q$ such that $\Lout(q,\xi \circ \tau_a,q_1) \not= \emptyset$ an automaton for $L_{q_1}$ on $z$ followed by the output produced in the simulation of $S$. During this simulation, $S'$ does not produce any output. As observed earlier, for some $q_1$,  the automaton for $L_{q_1}$ will eventually reach an accepting state. In this transition, $S'$ produces an output string $v''$ in $\Lout(q,\xi \circ \tau_a,q_1)$ and then continues by simply copying the remaining output of $S$.
\end{proof}


\subsubsection*{The strategy construction}



Finally, we explain how to construct $f_\tra$ such that (Inv0)--(Inv3) are ensured. 

The initial memory state is $[(q_0, \varepsilon, q_0^\dom, \varepsilon, q_0^\dom), (\varepsilon,\emptyset)]$. Then (Inv0)--(Inv3) are all satisfied:
\begin{itemize}
\item (Inv0) obviously holds.
\item (Inv1) holds because $q_0^\dom$ is not in $F_\dom$ because each word accepted by $A_\dom$ has to end with $\dashv$.
\item Since $R_{q_0}^\varepsilon = R_\tra$ and by assumption there is a sequential uniformizer for $R_\tra$, (Inv2) is satisfied.
\item (Inv3) is obviously satisfied by choosing $w = \varepsilon$ (because pumping the empty word results again in the empty word). 
\end{itemize}


Let $[(p,\rho,d',\xi,d);(u,M)]$ be the current memory state, $(p,\rho\xi,d)$ be the current position of the play, and assume that (Inv0)--(Inv3) are satisfied. Let $a \in \Sigmaend$ be the next move of Input leading to $(p,\rho\xi,d,a)$.

We now describe how $f_\tra$ selects the next moves of Output leading again to an Input vertex, and updates the memory. Later we verify that the invariant holds at the new Input vertex reached by the moves. For all cases, let $d_a = \delta_\dom(d,a)$.

\begin{enumerate}[(a)]
%\item If $p \in \Qin$, then $\rho\xi = \varepsilon$, $d' = d$, and $u=\varepsilon$. The only available move is (Out0), leading to $(p_1,\varepsilon,d_1)$ with $p_1 = \delta(p,a)$ and $d_1 = \delta_\dom(d,a)$. We update the memory to $[(p_1,\varepsilon,d_1,\varepsilon,d_1);(\varepsilon,\emptyset)]$. 
%
%for $p \in \Qout$ we show how to select the next move of Output such that the invariant is preserved. 
%\item If $|\rho| < K$ (and thus $\xi = u = x\varepsilon$, $d=d'$), then $f_T$ plays move (Out1) to $(p,\rho \circ \tau_a,d_1)$ with $d_1 = \delta_\dom(d,a)$, and updates the memory to $[(p,\rho,d_1,\varepsilon,d_1),(\varepsilon,\emptyset)]$.
\item Assume there is a $(p,\rho)$-uniformizer $S$ with $S(wa) \not= \varepsilon$ for all $w \in \Pump{|S|!}{(u,M)}$. Then the conditions of Lemma~\ref{lem:propagate-invariant} are satisfied. Let $q \in Q$ be the state with the properties from Lemma~\ref{lem:propagate-invariant}.

Let $w \in \Pump{|S|!}{(u,M)}$ such that $S(w) = \varepsilon$. The existence of $w$ is ensured by (Inv3) for the current node. 

We distinguish two cases depending on whether $a = \dashv$ or not.
  \begin{enumerate}[(1)]
  \item If $a \not= \dashv$, then play (Out2) with $v_{p,\rho,q}$, leading to vertex $(q,\xi,d,a)$, followed by the move (Out1) leading to $(q,\xi \circ \tau_a,d_a)$. 

Update the memory to $[(q,\xi \circ \tau_a,d_a,\varepsilon,d_a);(\varepsilon,\emptyset)]$.
  \item Assume $a = \dashv$ and $d_\dashv \in F_\dom$ (meaning that Input has played a string in the domain of $R_\tra$). In this case, the properties of $q$ are 
$\Lout(p,\rho,q) \not= \emptyset$ and $\dom(R_q^{\xi \circ \tau_\dashv}) = L(A_\dom,d_\dashv)$. Since  $L(A_\dom,d_\dashv) = \{\varepsilon\}$, the latter property implies that there is $r \in F$ with $\Lout(q,\xi \circ \tau_\dashv,r) \not= \emptyset$. So there must be $q'$ such that $\Lout(q,\xi,q') \not= \emptyset$ and $\Lout(q',\tau_\dashv,r) \not= \emptyset$.

Then $f_\tra$ plays (Out2) with $v_{p,\rho\xi,q'}$, leading to vertex $(q',\varepsilon,d,\dashv)$, followed by (Out0) with $v_{q',\tau_\dashv,r}$, leading to $(r,\varepsilon,d_\dashv)$. 

Update the memory to $[(r,\varepsilon,d_\dashv,\varepsilon,d_\dashv));(\varepsilon,\emptyset)]$.
  \end{enumerate}
\item Not case (a), and $\xi$ is not saturated. Then make the move (Out1) to $(p,\rho\xi \circ \tau_a,d_a)$.

Update the memory to $[(p,\rho,d',\xi \circ \tau_a,d_a);(ua,M)]$

This move is possible because $\xi = K$ would imply that $\xi$ is saturated  (Lemma~\ref{lem:length-saturated}).

\item Not case (a), and $\xi$ is saturated. Then there is a saturation witness $\xi = \xi_1\xi_2\xi_3$ with $\xi_3 = \varepsilon$. In particular, $M_3 = \emptyset$ for the  corresponding decomposition $(u,M) = (u_1,M_1)(u_2,M_2)(u_3,M_3)$ of $(u,M)$.
This means that $\xi_1\xi_2\xi_3 = \xi_1\xi_2$ is a saturation witness for $(u,M)$  as in Definition~\ref{def:safe-pump-word}. Then make the move (Out3) to $(p,\rho\xi_1\reduce{\xi_2},d,a)$ and update the memory to $[(p,\rho,d',\xi_1\reduce{\xi_2},d);(u,M')]$ with $M' = M \cup \{(|u_1|+1,|u_1|+|u_2|)\}$.
\end{enumerate}

\begin{lemma} \label{lem:invariant-preserved}
The strategy $f_T$ satisfies (Inv0)--(Inv3).
\end{lemma}
\begin{proof}
Most of the properties are obvious from the construction of the move:
\begin{itemize}
\item (Inv0) describes simple properties that directly follow from the construction of the new memory states. As only case we mention (Inv0)(iv). This follows from the fact that the move of type (Out3) is always applied when $\xi$ is saturated. This means if a new edge can be added to $(u,M)$ then it must involve the last letter that was added to $u$. Otherwise, the edge could have been added in a previous move.

\item (Inv1) clearly holds after (a)(2) by construction of the move. Furthermore, this is the only move after which the state of $A_\dom$ is in $F_\dom$.

\item (Inv2) holds after (b) and (c) because $p,\rho$, and $d'$ do not change. It holds after (a)(1) by Lemma~\ref{lem:propagate-invariant}. After (a)(2) the state of $A_\dom$ is in $F_\dom$ and hence (Inv2) is trivially satisfied.

\item (Inv3) is trivially satisfied after (a)(1) and (a)(2) because the new pump-word is $(\varepsilon,\emptyset)$. (Inv3) also holds after (b) because the new pump-word is $(ua,M)$ and the negation of (a) is exactly (Inv3) for $(ua,M)$. (Inv3) after (c) requires some more work, and is shown below.
\end{itemize}
We need to show that (Inv3) is preserved after an application of case (c) in the strategy description. So we need to show that for every $(p,\rho)$-uniformizer $S$ there is $w \in \Pump{|S|!}{(u,M')}$ such that $S(w) = \varepsilon$, where $M'$ extends $M$ by the new edge as defined in case (c).

Toward a contradiction, assume that there is $(p,\rho)$-uniformizer $S$ such that $S(w) = \varepsilon$ for all $w \in \Pump{|S|!}{(u,M')}$. We show that then there also exists a $(p,\rho)$-uniformizer $S'$ such that $S(w) = \varepsilon$ for all $w \in \Pump{|S'|!}{(u,M)}$, contradicting the assumption that (Inv3) holds for $(u,M)$. 

We construct $S'$ such that $|S'| \ge |S|$ and $S(w) = \varepsilon$ for all $w \in \Pump{|S|!}{(u,M)}$, which then implies $S(w) = \varepsilon$ for all $w \in \Pump{|S'|!}{(u,M)}$.

Let $\xi = \xi_1\xi_2\xi_3$ and $(u,M) = (u_1,M_1)(u_2,M_2)(u_3,M_3)$ be as in case (c). Recall that $\xi_3 = \varepsilon$ and thus $u_3 = \varepsilon$,  $\xi = \xi_1\xi_2$, and $(u,M) = (u_1,M_1)(u_2,M_2)$
%Words in $\Pump{|S|!}{(u,M')}$ are thus of the form $w_1(w_2)^\ell$ with  $w_1 \in \Pump{|S|!}{(u_1,M_1)}$ and $w_2 \in \Pump{|S|!}{(u_2,M_2)}$.

We describe how $S'$ works in two phases. We do not provide a formal definition of $S'$ because it should be clear that the description below can be implemented by a sequential finite state transducer.
\begin{itemize}
\item In the first phase, $S'$ mimics  $S$ on the input, while at the same time simulating an automaton for $\Pump{|S|!}{(u_1,M_1)}$. If during this phase $S$ produces output, $S'$ simply continues to mimic $S$ and cancels all other activities (recall that the goal is construct a transducer $S'$ that produces output on all strings from $\Pump{|S|!}{(u,M)}$; so if $S$ produces output we are done for this input string).

If $S'$ detects that $w_1 \in \Pump{|S|!}{(u_1,M_1)}$ has been read (and no output has been produced), jump to the next phase.

\item Let $s_1$ be the state of $S$ with $S:s_0 \xrightarrow{w_1/\varepsilon} s$ (which is reached during the simulation of $S$ in the first phase). Fix some $w_2 \in \Pump{|S|!}{(u_2,M_2)}$, e.g., the shortest word in this set. Let $h \ge 0$ be maximal such that starting from $s_1$, $S$ does not produce any output on $(w_2)^h$. Note that there exists a maximal such $h$ because $S$ will produce output for $|S|!$ repetitions of $w_2$. So the situation is now as follows:
\[
S: s_0 \xrightarrow{w_1 / \varepsilon} s_1 \xrightarrow{(w_2)^h / \varepsilon} s_1'
\]

In the second phase, $S'$ continues the simulation of $S$ but now from state $s_1'$. If the first output in this simulation of $S$ is produced, it is of the form $yz$ with $y \in \Lout(p,\rho,q)$ for some state $q$. Then, $S'$ outputs $y$ and jumps to the third phase.
\item The current situation can be depicted as follows, where the second line only indicates the part of $S'$ that simulates $S$:
\[
  \begin{array}{l}
S: s_0 \xrightarrow{w_1 / \varepsilon} s_1 \xrightarrow{(w_2)^h / \varepsilon} s_1' \xrightarrow{w'/yz} s_2 \\    
S': s_0 \xrightarrow{w_1 / \varepsilon} s_1 \leadsto s_1' \xrightarrow{w'/y} s_2
  \end{array}
\] 
Note that the actual input is $w_1w'$, and that $(w_2)^h$ has only virtually be inserted in the computation of $S$.

For the third phase, let $L_{\text{Pump},{s_1}'}$ be the set of all $\hat{w} \in \Pump{|S|!}{(u_1,M_1),(u_2,M_2)^h}$ with $S: s_0 \xrightarrow{\hat{w}/\varepsilon} s_1'$. Note that $w_1(w_2)^h$ is such a word, and that $L_{\text{Pump},{s_1}'}$ is regular.

In the third phase, $S'$ continues the simulation of $S$ from $s_2$ but without producing output. Instead, it waits until the output that $S$ would have produced, including the pending $z$ from the previous transition, contains a prefix $\hat{v} \in \Lout(q,\rho_{\hat{w}},r)$ for some $r$ and some $\hat{w} \in L_{\text{Pump},{s_1}'}$ such that $\Lout(q,\xi_1(\xi_2)^h,r) \not= \emptyset$. If such a prefix $\hat{v}$ is reached, then $S'$ outputs instead a word $v_1 \in \Lout(q,\xi_1,r)$, which exists because $P_{\xi_1} = P_{\xi_1}P_{\xi_2} \cdots P_{\xi_2}$. And after that, $S'$ just copies the output of $S$.
\end{itemize}


We need to argue that $S'$ is a $(p,\rho)$-uniformizer with the desired property, and  for the third phase, that the output of $S$ contains such a prefix $\hat{v}$ that can be substituted by $v_1 \in \Lout(q,\xi_1(\xi_2)^h,r)$.

For this purpose, let $x$ be an input that takes $S$ from $s_2$ into a final state $s_3$, and let $v$ be the corresponding output. The whole computation of $S$ that is used in the description above looks as follows:
\[
S: s_0 \xrightarrow{w_1 / \varepsilon} s_1 \xrightarrow{(w_2)^h / \varepsilon} s_1' \xrightarrow{w'/yz} s_2 \xrightarrow{x/v} s_3    
\]
We note that by definition of $R_\rho^p$, the pair $(w_1(w_2)^hw'x,zv)$ is accepted by $\tra$ from state $q$. Now assume that $zv = \hat{v}v'$ has a prefix $\hat{v}$ as described in the third phase. Then we can replace $w_1(w_2)^h$ in the above computations of $S$ by $\hat{w}$:
\[
S: s_0 \xrightarrow{\hat{w} / \varepsilon} s_1' \xrightarrow{w'/yz} s_2 \xrightarrow{x/v} s_3    
\]
and we thus know that $(\hat{w}w'x,\hat{v}v')$ is accepted by $T$ from $q$, and furthermore $\delta^*(q,\hat{w},\hat{v}) = (r,\varepsilon,\varepsilon)$ (for $r$ as in the third phase). By the choice of $v_1 \in \Lout(q,\xi_1,r)$ and the fact that $w_1$ is compatible with $\xi_1$, we obtain that $\delta^*(q,w_1,v_1) = (r,\varepsilon,\varepsilon)$.

The computation of $S'$ can be sketched  as follows (again only showing the states of the simulation of $S$ inside $S'$):
\[
S': s_0 \xrightarrow{w_1 / \varepsilon} s_1 \leadsto s_1' \xrightarrow{w'/y} s_2  \xrightarrow{x/v_1v'} s_3 
\] 
Since $\delta^*(q,w_1,v_1) = (r,\varepsilon,\varepsilon)$, we obtain that $(w_1w'x,v_1v')$ is accepted by $\tra$ from $q$. Hence $S'$ is indeed a $(p,\rho)$-uniformizer.

It remains to prove the existence of the prefix $v_1$ in the output $zv$.
Let us verify by applying  Lemma~\ref{lem:output-large-pumping} that the output must contain such a prefix.



Because the pumping factors for $w_1$ and $w_2$ are at least $|S|!$, one can safely pump the factors further by multiples of $|S|!$ without $S$ noticing the difference. Hence, for each $k$ one can find some $\hat{w} \in \Pump{k}{(u_1,M_1)(u_2,M_2)^h}$ with $S:s_0 \xrightarrow{\hat{w}/\varepsilon} s_1'$.
Thus, there is a prefix $v'$ of $zv$ and some  $\hat{w} \in \Pump{3|v'|}{(u_1,M_1)(u_2,M_2)^h}$ with $v' \in \Lout(q,\rho_{\hat{w}},r)$ for a state $r$. Then Lemma~\ref{lem:output-large-pumping} yields that $\Lout(q,\xi_1(\xi_2)^h,r) \not= \emptyset$.
\end{proof}

Lemma~\ref{lem:drat-uniformizer-to-strategy} now follows from
Lemma~\ref{lem:invariant-implies-winning} and
Lemma~\ref{lem:invariant-preserved}.


==> On Equivalence and Uniformisation Problems for Finite Transducers/drat.tex <==
\vspace{-1em}
\section{Deterministic Rational Transductions} \label{sec:drat}

In this section we consider another subclass of rational
transductions, namely the deterministic rational transductions,
denoted by DRat. This class is defined in terms of specific
deterministic transducers and some problems that are undecidable for
general rational transductions are decidable in the case of DRat. For
example, the equivalence problem is decidable \cite{Bird73} (while
inclusion is easily seen to be undecidable \cite{FischerR68}), and
whether a given relation in DRat is recognisable \cite{CartonCG06} is
also decidable.
We obtain here another decidability result, namely that the sequential
uniformisation problem is decidable for deterministic transducers. 

For the definition of deterministic rational transducers, we work with
endmarkers (this is the common way of doing it, see also \cite{DBLP:books/daglib/0023547}). The determinism includes the standard definition of unique
successor states for each symbol and additionally a deterministic
choice between input and output. This is enforced by a partition of
the state space into states processing input symbols and states
processing output symbols.

\begin{figure}[t]
\begin{center}
\begin{tikzpicture}[->,>=stealth',auto,node
    distance=1cm,thick,scale=0.7,every node/.style={scale=0.7}]
  \tikzstyle{every state}=[fill=yellow!30,text=black]
  % \tikzstyle{every edge}=[draw=black,text=red]
  \tikzstyle{initial}=[initial by arrow, initial where=left, initial text=]
  \tikzstyle{accepting}=[accepting by arrow, accepting where=right, accepting text=]
  \tikzstyle{acceptingdown}=[accepting by arrow, accepting where=below, accepting text=]

  \tikzstyle{initialT1}=[initial by arrow, initial where=left, initial
  text=]

  \node[initialT1,state] (A) at (0,0) {};
  \node[state]           (B) at (2,0) {};
  \node[state]           (C) at (4,0) {};
  \node[state]           (D) at (6,0) {};
  \node[state,accepting] (E) at (8,0) {};
  \node[state]           (F) at (2,2) {};
  \node[state]           (G) at (2,-2){};
  
  \path (A) edge [loop above] node {$\begin{array}{l}\trans{a}{\epsilon}\\\trans{b}{\epsilon}\end{array}$} (A);
  \path (A) edge node {\trans{\#}{\epsilon}} (B);
  \path (B) edge node {\trans{\#}{\epsilon}} (C);
  \path (B) edge [bend left] node {\trans{a}{\epsilon}} (F);
  \path (B) edge [bend right,swap] node {\trans{b}{\epsilon}} (G);
  \path (C) edge [loop above] node {$\begin{array}{l}\trans{a}{\epsilon}\\\trans{b}{\epsilon}\end{array}$} (C);
  \path (C) edge node {\trans{\dashv\ }{\epsilon}} (D);
  \path (D) edge [loop above] node {$\begin{array}{l}\trans{\epsilon}{a}\\\trans{\epsilon}{b}\end{array}$} (D);
  \path (D) edge node {\trans{\epsilon }{\ \dashv}} (E);
  \path (F) edge [bend left] node {\trans{\epsilon}{a}} (B);
  \path (G) edge [bend right,swap] node {\trans{\epsilon}{b}} (B);
\end{tikzpicture}
\vspace{-2em}
\end{center}
\caption{A deterministic transducer with endmarker for $\mathcal R_1$ from Ex.~\ref{ex:drat}.}
\vspace{-1em}
\label{fig:drat} 
\end{figure}

\begin{example}\label{ex:drat}
 The transduction $\mathcal R_1 = \{ (u\#v\#w,vx) \mid u,v,w,x \in \{a,b\}^*\}$ is in DRat since it is recognised by the deterministic transducer depicted in Fig.~\ref{fig:drat} over the alphabet 
 $\{a,b,\#\}$ with endmarker $\dashv$. Note that for each state the outgoing transitions
 either all have $\epsilon$ as  output component, or all have
 $\epsilon$ as input component. In the formal definition, this
 is captured by the partition into input and output states. 
\end{example}

Let $\Sigma$
be an alphabet and $\dashv$
a fresh symbol used as endmarker. We let
$\Sigmaend := \Sigma \cup \{\dashv\}$.
A deterministic transducer over the alphabet $\Sigma$
with endmarker $\dashv$
is of the form $\tra = (\Qin,\Qout,F,q_0,\delta)$
with a set $\Qin$
of input states, a set $\Qout$
of output states (we write $Q$
for the union of these two sets), a unique initial state $q_0$,
a transition function
$\delta: Q \times \Sigmaend \rightarrow Q$,
and a set $F \subseteq Q$
of accepting states. In the presence of endmarkers, the final output function is not required anymore.

For defining the semantics of such a deterministic transducer, one can transform it into a standard transducer. However, this transformation needs to take care of the endmarker only being allowed at the end of the word, which is not enforced in the definition of deterministic transducers. To avoid this, we rather define the semantics by extending the transition function to pairs of words (input and output word).
For $(u,v) \in \Sigmaend^* \times \Sigmaend^*$
and $q \in Q$,
we define
$\delta^*: Q \times \Sigmaend^* \times \Sigmaend^* \rightarrow Q
\times \Sigmaend^* \times \Sigmaend^*$ inductively as follows:
\begin{itemize}
\item If $q \in \Qin$, then $\delta^*(q,\epsilon,v) =
  (q,\epsilon,v)$ and $\delta^*(q,au,v) =
  \delta^*(\delta(q,a),u,v)$.
\item If $q \in \Qout$, then $\delta^*(q,u,\epsilon) =
  (q,u,\epsilon)$ and $\delta^*(q,u,av) = \delta^*(\delta(q,a),u,v)$.
\end{itemize}
So $\delta^*$
applies $\delta$
to the next input letter from states in $\Qin$
and to the next output letter from states in $\Qout$
as long as possible. The transduction $\rel{\tra}$
defined by $\tra$ is
\[
  \rel{\tra} = \{(u,v) \in \Sigma^* \times \Sigma^* \mid
  \delta^*(q_0,u\dashv,v\dashv) = (q,\epsilon,\epsilon) \mbox{
    with } q \in F\}.
\]
Recall from Section~\ref{sec:fvalued} that $k$-delay inclusion and
equivalence are
complete for finite-valued transducers, as stated in
Theorem~\ref{lem:finitelyambiguous}. We note that this is not the case
for DRat. 
\begin{remark}
  There are deterministic transducers $\tra_1$ and $\tra_2$ such that
  $\tra_1 \equiv \tra_2$ but there is no $k$ such that $\tra_1 \equiv_k \tra_2$.
\end{remark}
\begin{proof}
  Consider the complete relation $\Sigma^* \times \Sigma^*$,
  and let $\tra_1$
  be the deterministic transducer that first reads all input symbols
  (up to the endmarker $\dashv$),
  and then reads all output symbols. Let $\tra_2$
  be the deterministic transducer that first reads all output symbols
  and then the input symbols. Obviously,
  $\rel{\tra_1} = \rel{\tra_2} = \Sigma^* \times \Sigma^*$.
  However, the lag for the two runs of $\tra_1$,
  $\tra_2$ on a pair $(u,v)$ is $|v|$ and thus not bounded.
\end{proof}

Our main result for DRat is the following, which extends the corresponding
result for automatic relations from \cite{CarayolL14}.
\begin{restatable}{theorem}{dratunif}\label{the:drat-unif}
 The sequential uniformisation problem for deterministic transducers is decidable. 
\end{restatable}
The proof uses the game-theoretic approach, building a game between
players Input and Output. A winning strategy for player Output then
corresponds to a sequential uniformiser. The moves of the game simulate the deterministic transducer $T$ on the pairs of input and output word played by the two players in order to check whether the output indeed matches the input. However, Output might need to delay the moves to gain some lookahead on the input for making the next decisions. The main challenge in the proof is to find a way to keep the lookahead information bounded without losing too much information. It is not sufficient to simply store words of bounded length as lookahead. The information in the lookahead rather provides information on the behaviour that the lookahead word induces in $T$. Player Output can delete parts of this information to reduce the size of the lookahead. 


The sequential uniformiser that is constructed from the game in the
decidability proof can be shown to have bounded delay. So we obtain
the following result, showing that sequential $k$-uniformisation is complete for deterministic transducers. 

\begin{restatable}{theorem}{dratkdelay}\label{the:drat-k-delay}
    Any sequentially uniformisable deterministic transducer is
    sequentially $k$-uniformisable for some $k\in \mathbb{N}$ that can be computed from the given transducer.
\end{restatable}


%%% Local Variables:
%%% TeX-master: "main"
%%% End:

==> On Equivalence and Uniformisation Problems for Finite Transducers/fvalued.tex <==
\section{Finite-valued transducers}\label{sec:fvalued}


Let $m\in\mathbb{N}$. We remind the reader that a transducer $\tra$ is called
\textit{$m$-valued} if each input has at most $m$ outputs, i.e. for
all $w\in\dom(\tra)$, $|\rel{\tra}(w)|\leq m$. It is finite-valued if
it is $m$-valued for some $m$. Finite-valuedness is decidable
\cite{DBLP:journals/acta/Weber89}. We prove that for the class of
finite-valued transducers, $k$-inclusion and sequential $k$-uniformisation
are complete. This yields, for finite-valued transducers, an alternative proof of the decidability of
the inclusion problem, and a new result: The decidability of
sequential uniformisation. 


Let $m$ be a natural number. An automaton $A$ (resp. transducer
$\tra$) is called $m$-ambiguous if it is real-time\footnote{For
  simplicity reasons, we put real-timeness in the definition, but it
  is known to be wlog.}, and for any word $w\in
\lang{A}$ (resp. $w\in \dom(\tra)$), there exist at most $m$
accepting runs of $A$ (resp. $\tra$) on $w$.
An automaton (transducer) is called finitely ambiguous if there exists
$m \in \mathbb{N}$ such that it is $m$-ambiguous, and unambiguous if
it is $1$-ambiguous. Our proofs uses the following known decomposition
initially due to Weber:
\begin{theorem}\label{trans_fv}
\cite{DBLP:conf/mfcs/Weber88,journals/mst/SakarovitchS10} Any finite-valued transducer $\tra$ is
(effectively) equivalent to a union of unambiguous transducers. 
\end{theorem}





%% caution: it would not be correct to say that T is n-ambiguous if
%% its input automaton is. It would be correct if we impose that for
%% any two transitions (q,a,w1,p), (q,a,w2,p') implies p \neq p'

We first prove that, for the class of finitely ambiguous transducers,
inclusion and equivalence reduces to $k$-inclusion and $k$-equivalence
for some computable $k$. We state this result for inclusion, which immediately
implies it for equivalence.
% Proposition \ref{prop:notcomplete} does not hold for inclusion and equivalence.

\begin{restatable}{theorem}{thmfinitelyambiguous}\label{lem:finitelyambiguous}
Let $\tra_1$ and $\tra_2$ be two real-time transducers such that $\tra_2$ is $m$-ambiguous. 
Then there exists a computable integer $k$ such that $\tra_1\subseteq
\tra_2 \implies \tra_1\subseteq_k \tra_2.$ Moreover, $k$ can be chosen to be exponential in the size of $\tra_2$
and linear in the size of $\tra_1$.
\end{restatable}

\begin{proof}[Sketch of Proof]

We show the result by choosing $k$ high enough with respect to the size of $\tra_1$ and $\tra_2$, assuming that $\tra_1$ is not $k$-included
    in $\tra_2$, and exhibiting a contradiction.
If $\tra_1$ is not $k$-included
    in $\tra_2$, there exists a word $w\in \lang{\tra_1}$ such that for all words
    $w'\in \lang{\tra_2}$ equivalent to $w$, $\lag(w,w')>k$.
    Such a word is called a \textit{witness}.
    Given a witness $v$, let $N_{\tra_2}(v)$ denote the number of words $v'\in\lang{\tra_2}$
    equivalent to $v$.
We prove that for each witness $v$, if $N_{\tra_2}(v) > 0$, there exists a witness
      $t\in\lang{\tra_1}$ such that $N_{\tra_2}(t)<N_{\tra_2}(v)$,
      which by induction yields a contradiction. To do so, we follow three steps.

$(i)$ We exhibit synchronised loops between the run $\rho$ of $\tra_1$ recognising $v$, and the set $R_2$ containing all the runs of $\tra_2$ recognising words equivalent to $v$.

$(ii)$ Given a run $\rho' \in R_2$, as the delay between $\rho$ and $\rho'$ is greater than $k$ at some point, we can chose one of those loops such that the delay between $\rho$ and $\rho'$ grows along the loop.

$(iii)$ By iterating the loop a sufficient number of times, we
generate a new witness $t$ such that $N_{T_2}(t)<N_{T_2}(v)$.

Then, as $\tra_2$ is $m$-ambiguous, if there exists a witness $w$, $N_{\tra_2}(w) \leq m$, and, by applying the preceding remark inductively, we expose a witness $w_0$ such that $N_{\tra_2}(w_0) = 0$.
In other words,
$(\pi_{\inp}(w_0),\pi_{\outp}(w_0))\in\rel{\tra_1}\cap
\overline{\rel{\tra_2}}$, which contradicts the fact that $\rel{\tra_1}\subseteq
\rel{\tra_2}$.
\end{proof}

Since $k$-inclusion is decidable by Theorem \ref{thm:rat},
Theorem \ref{lem:finitelyambiguous} implies that the inclusion and
equivalence problems are decidable for finitely ambiguous
transducers. From the decomposition of Theorem \ref{trans_fv}, we
obtain an alternative proof of the decidability of equivalence of
finite-valued transducers, which was proved in \cite{CulKar86c,DBLP:conf/mfcs/Weber88}. 

\begin{corollary}[\cite{CulKar86c,DBLP:conf/mfcs/Weber88} Alternative proof]
The inclusion and equivalence problems for finite-valued transducers are decidable.
\end{corollary}

We now prove the two corresponding results for the sequential uniformisation problem.

\begin{restatable}{theorem}{thmunifvalued}\label{f_a_det}
Let $\tra$ be a real-time trim transducer given as a finite union of unambiguous transducers.
Then there exists a computable integer $N_T$ such that if $\tra$ is
sequentially uniformisable, then it is sequentially $N_T$-uniformisable.
\end{restatable}

\begin{proof}[Sketch of proof]
If $\tra$ is seq-uniformisable, then there exists a sequential uniformiser $\uni$
    of $\tra$ such that
    $\dom(U) = \dom(T)$ and $U\subseteq T$. The latter inclusion implies, by Theorem
    \ref{lem:finitelyambiguous}, that there exists an integer $k$ such
    that $\uni\subseteq_k T$, and so $\uni$ is a seq-$k$-uniformiser of $\tra$.
    However, $k$ depends on the number of states of the hypothetical
    uniformiser $\uni$. We show how to construct, by simulating the
    behaviour of $U$, another  seq-$N_T$-uniformiser $U'$, where $N_T$ only depends on
    $T$ and can be computed. 


    More precisely, we define a function $\rho : \Sigma^*\rightarrow
    \Sigma^*$ and define $U'$ such that on any input $w$, it simulates $U$ on 
    input $\rho(w)$. The function $\rho$ iterates some well-chosen
    subwords of $w$  to blow up the delay between the outputs of the
    runs of $T$ on $\rho(w)$. On input $\rho(w)$, any seq-$k$-uniformiser of
    $T$, and $U$ in particular, is forced to make choices between
    possible outputs of $T$ on $\rho(w)$, in
    order to decrease the delay. % 
 % in order to blow up the delay between $U$ and $T$ on
    % input $\rho(w)$ (up to $k$ as $U$ is a seq-$k$-uniformiser of
    % $T$). This blow-up only happens when on $w$, the delay between
    % $U$ and $T$ is close to $N$.
 The main idea is that if, by making
    some good choice of output, 
    $U$ is able to react to a threat of exceeding delay $k$ on
    $\rho(w)$, then by doing the
    same choice on $w$, $U'$ can also react to a threat of exceeding
    delay $N_T$. 



    We identify several key properties that $\rho$ must satisfy, in
    order to be able to construct $U'$. For instance, we require that
    $\rho(w)$ is a prefix of $\rho(wa)$ for all $w\in\Sigma^*$,
    $a\in\Sigma$, but also some property relating the delays between
    $U$ and $T$ on  input $w$ and on input $\rho(w)$. 



    The challenging part of the proof is to prove the existence of $N_T$ and
    $\rho$. It is based on a study of the structural properties of
    the transition monoid of finitely ambiguous transducers (a monoid
    that captures the state behaviour of automata and transducers),
    and the effect of its elements on the delays. In particular,
    subwords of $w$ that are iterated to define $\rho(w)$ correspond to idempotent
    elements in the transition monoid of $T$, and the bound $N_T$ is
    obtained by an application of Ramsey's theorem.
\end{proof}


Since by Theorem~\ref{thm:rat} every finite-valued transducer is
effectively equivalent to a finitely ambiguous transducer, the
sequential uniformisation problem for finite-valued transducers reduces to sequential
$N$-uniformisation, for computable integers $N$. Hence by Theorem
\ref{thm:rat} and the fact that any transducer can be trimmed in
polynomial time, we get decidability of sequential uniformisation of
finite-valued transducers, one of the main results of this paper. 

% This proves that for every transducer $\tra$ given as a union of
% unambiguous transducers, the uniformisation problem reduces to the
% $N$-delay uniformisation problem for a computable $N$, which is
% decidable, by Theorem \ref{thm:rat}.
% Once again, as any finite-valued transducer can be transformed into an
% equivalent union of unambiguous transducers, based on Theorem
% \ref{trans_fv}, we have the following corollary.

\begin{corollary}\label{fv_unif}
The sequential uniformisation problem for finite-valued
transducers is decidable.
\end{corollary}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> On Equivalence and Uniformisation Problems for Finite Transducers/intro.tex <==
\section{Introduction}

Transductions generalise finite word languages to binary relations of
finite words. The notion of rationality for languages, and its
correspondence with finite automata, has been extended to transductions
and finite automata over pairs of words, called \emph{finite transducers}
\cite{berstel2009}. In this paper, we study decision problems for
finite transducers and prove new decidability results. 


\vspace{1mm}
\noindent\textbf{Finite transducers} (Finite) transducers are
nondeterministic finite
automata whose transitions are labelled by pairs of words. The
(rational) transduction $\rel{\tra}$ defined by a transducer $\tra$ consists of all the pairs of
words $(u,v)$ obtained by concatenating the pairs occurring on
transitions of its successful computations. In this paper, we follow a
dynamic vision of transducers, as a machine that processes input words $u$
and produces output words $v$. Therefore, we may speak of the domain
of a transduction, as the language of input words that admit at least
one output word. 


\vspace{1mm}\noindent\textbf{Equivalence problem} Unlike finite
automata, finite transducers have undecidable inclusion and equivalence problems
\cite{DBLP:journals/jacm/Griffiths68,FischerR68}, even restricted to unary
alphabets \cite{SICOMP::Ibarra1978}. The largest known classes with
decidable equivalence problem are those of finite-valued transducers
and deterministic transducers. A transducer is finite-valued if it
produces at most $k$ outputs per input, for a bound $k$
that only depends on the transducer. It is decidable whether a
transducer is $k$-valued for a given $k$ \cite{GurIba83}, and whether there
exists $k$ such that it is $k$-valued \cite{DBLP:journals/acta/Weber89}. Any finite-valued
transducer is known to be (effectively) equivalent to a finite union of unambiguous 
transducers \cite{DBLP:conf/mfcs/Weber88}, and thus to a finitely ambiguous transducer. 
Equivalence of $k$-ambiguous transducers was shown to be
decidable in \cite{GurIba83}, and equivalence of $k$-valued
transducers was first shown to be decidable in
\cite{CulKar86c,DBLP:conf/mfcs/Weber88}. Other algorithms with better
complexities appeared later, and the best known algorithm runs in
exponential time, for a fixed $k$ \cite{DBLP:conf/dlt/Souza08}.  

A transducer is deterministic if the transitions are deterministic in
the classical sense, and furthermore each state  processes either only
input symbols or only output symbols. The class of deterministic
rational transductions is also referred to as DRat, and it strictly
extends the class of synchronous rational transductions (also called
automatic relations), see e.g.\ \cite{CartonCG06} for an overview of
these sub-classes of rational transductions. As opposed to the
class of finite-valued transducers, it is undecidable whether a
transduction is equivalent to a deterministic transduction
\cite{FischerR68}. However, the equivalence problem for DRat is known
to be decidable \cite{Bird73}, even in polynomial time
\cite{FriedmanG82}. This makes this class an interesting candidate for
further investigations of decision problems.

\vspace{1mm}
\noindent\textbf{Uniformisation problem} Two classes of interest are
the rational and sequential functions, which are respectively defined
by $1$-valued transducers and sequential transducers. The latter read 
input words in a deterministic manner, and therefore produce a unique output word for each
input. There are rational functions that are not sequential, but it is
decidable in \textsc{PTime} whether a transducer defines a sequential
function \cite{DBLP:journals/iandc/WeberK95}. Since rational transductions do not define, in general,
functions, an interesting question is whether a unique output word can
be picked for each input word of a rational transduction $R$, in a
regular way, thus defining a function $f\subseteq R$ with the same
domain as $R$. Such a function $f$ is called a \emph{uniformiser} of $R$. 
It is known that any rational transduction admits a rational uniformiser
\cite{journals/iandc/Kobayashi69,Eilenberg:1974:ALM:540337} and, in
the case of DRat, even a \emph{lexicographic} uniformiser that picks the
smallest output words according to a lexicographic order, making the
uniformiser only depend on the transduction \cite{lncs194*300,PelSak99}.
In this paper, we are interested in sequential uniformisers. Even rational functions do not admit
sequential uniformisers in general, and therefore this gives rise to a
decision problem: Given a finite transducer, does it admit a
sequential uniformiser? It is worth noting that even if any rational
transduction $R$ can be uniformised by a rational uniformiser $U$, the
sequential uniformisability of $R$ does not imply, in general, that
\emph{any} of the uniformisers $U$ is equivalent to a sequential transducer. As a matter of fact, it
is known that the sequential uniformisation problem is undecidable for
rational transductions~\cite{CarayolL14}. 



The sequential uniformisation problem echoes a similar problem introduced by
Church, the \emph{synthesis problem}, which currently receives a
lot of attention from the computer-aided verification community in the
context of open reactive systems (see
\cite{KupfermanPV06,FiliotJR11,BloemJPPS12} for some work on this
subject from the last decade). This problem asks whether given a logical
specification of a system, there exists an implementation that
satisfies it. In this context, reactive systems are non-terminating
systems that react to some unpredictable environment stimuli in a
\emph{synchronised} fashion: for each environment input, they produce
an output in a deterministic manner, such that the specification is met in the limit. 
Their executions are modelled by infinite words over a
product alphabet, and the interaction with the environment makes 
game theory a powerful tool in this context. A seminal result due to B\"uchi and Landweber shows
that the synthesis problem is decidable for MSO specifications
\cite{BuLa69} (see \cite{Thomas08} for a modern presentation and an
overview). 

Restricted to finite words, the sequential uniformisation problem generalises the synthesis
problem to an asynchronous setting: the transduction $R$ is the specification,
while the sequential uniformiser $f$ is the implementation.
%, and both are allowed to produce several outputs per input, or none. 

% Unlike finite automata, important problems are undecidable for finite
% transducers. The inclusion and equivalence problems asks whether given
% two transducers $\tra_1$ and $\tra_2$, the transductions they define
% are included and equal respectively. These problems are undecidable
% \cite{DBLP:journals/jacm/Griffiths68}. Large subclasses of rational
% transductions have then been introduced to recover decidability of
% inclusion and equivalence. The largest known class of 


\vspace{1mm}
\noindent\textbf{Resynchronisers} One of the main difficulty of
transducers is that two equivalent transducers may produce their
outputs very differently: One transducer may go fast and be ahead of
the other. By tagging symbols with two colours (for input and output),
transductions can be seen as languages, called \emph{synchronisation
languages}. It is known by
Nivat's theorem that rational transductions are synchronised by
regular languages \cite{Niv-transductions-lc}, and any transducer defines a
regular synchronisation language. Other correspondences between classes of
synchronisation languages and classes of rational transductions have
been established in \cite{conf/stacs/FigueiraL14}.
However in general, there is an infinite number of synchronisation
languages for a single transduction, making problems such as equivalence and sequential
uniformisation undecidable. To overcome this difficulty, Bojanczyk has
introduced \emph{transductions with origin information}, which amounts
to add the synchronisation information into the semantics of
transducers, via an origin function mapping output positions their
originating input positions \cite{DBLP:journals/corr/Bojanczyk13}. The main result of
\cite{DBLP:journals/corr/Bojanczyk13} is a
machine-independent characterisation of transductions (with origin
information) defined by two-way transducers. With respect to the
equivalence problem, considering the origin information makes the
problem easy: two transducers define the same transduction with
same origin mappings if they have the same synchronisation language. 
In this paper, we generalise this idea and propose decision problems modulo resynchronisation. A
\emph{resynchroniser} $\sync$ is a transduction, mapping a synchronisation
language to another one. Then, we consider related equivalence and
sequential uniformiser problems: for instance, given two transducers, are their
synchronisation languages equal modulo $\sync$? For the identity
resynchroniser, it is the same as origin-equivalence.


\vspace{1mm}
\noindent\textbf{Contributions} As a first contribution, we show that
inclusion, equivalence and sequential uniformisation are decidable
modulo \emph{rational} resynchronisers. For equivalence, it easily
reduces to an automata equivalence problem. For sequential
uniformisation, it boils down to solving a two-player safety game. 
We then consider a particular class of resynchronisers, the
\emph{$k$-delay resynchronisers}, that can apply a fixed delay $k$ 
to a synchronisation language, where the delay is a measure of how
ahead an output word is from another one \cite{BealCPS03}. The $k$-delay
resynchroniser is rational for each $k$, which implies the decidability of the
corresponding decision problem. Interestingly, we show that for the
class of real-time transducers (reading at least one input symbol in
each transition),
$k$-delay resynchronisers encompass all the power of rational
synchronisers with respect to the decision problems considered in this
paper. 

Our second main contribution is to show that equivalence and
sequential uniformisation modulo $k$-delay resynchronisers are
complete for finite-valued transducers. Given two finite-valued
transducers, if they are equivalent, then some $k$ can be computed 
such that they are $k$-delay equivalent. This yields another, delay-based, proof of
the decidability of finite-valued transducer equivalence. We show a
similar result for sequential uniformisation, by a pumping argument
based on an analysis of the idempotent elements in the transition
monoid of finitely-ambiguous transducers. This implies a new result: The decidability of
sequential uniformisation for finite-valued transducers. 


Finally, our third main contribution is a decidability proof for the
sequential uniformisation problem for deterministic rational
transductions, extending a corresponding result for automatic
relations from  \cite{CarayolL14}.


\vspace{1mm}
\noindent\textbf{Structure of the paper} In Section~\ref{sec:prelims},
we introduce automata, transducers and decision problems for them. In
Section~\ref{sec:synch}, we define the notion of resynchronisers for
transductions and study their associated decision problems. We also
introduce the particular class of bounded delay resynchronisers. In
Section \ref{sec:fvalued}, we study the class of finite-valued
rational transductions and prove decidability of their sequential
uniformisation. Finally in Section \ref{sec:drat}, we prove
decidability of sequential uniformisation for deterministic rational
transductions. Due to lack of space, proofs are only sketched in the
paper. All full proofs can be found in the appendix section. 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> On Equivalence and Uniformisation Problems for Finite Transducers/macro.tex <==

\newcommand\sem[1]{\llbracket #1 \rrbracket}
\newcommand\inter[1]{\llbracket #1 \rrbracket}
\newcommand\interorigin[1]{\llbracket #1 \rrbracket_{\mathcal{O}}}
\newcommand\trans[2]{\ensuremath{#1\mid #2}}
\newcommand\origin[1]{R_{#1}}
\newcommand\oporigin[1]{R'_{#1}}
\newcommand\delay{\Delta}
\newcommand\aut{A}
\newcommand\tra{T}
\newcommand\uni{U}
\newcommand\sync{\mathbb{S}}
\newcommand\dsync{\mathbb{D}}
\newcommand\eof{\hfill$\square$}
\newcommand\inp{\mathbbmtt{i}}
\newcommand\outp{\mathbbmtt{o}}
\newcommand\dom{\text{dom}}
\newcommand\id{\text{id}}

\newcommand\inr{\text{in}}
\newcommand\outr{\text{out}}

\newcommand\del{\text{delay}}
\newcommand\lag{\text{lag}}

% \newcommand\lag[2]{\textup{LAG}(#1,#2)}

\newcommand{\manu}[1]{\marginpar{Manu:#1}}
\newcommand{\isma}[1]{\quad\\\fbox{\parbox{\linewidth}{{\sc Isma\"el}:\\#1}}}
\newcommand{\todo}[1]{\quad\\\fbox{\parbox{\linewidth}{{\sc TODO}:\\#1}}}

\newcommand{\lang}[1]{\mathcal{L}_{#1}}
\newcommand{\rel}[1]{\mathcal{R}_{#1}}

\newcommand\alphab{\Sigma}
\newcommand\ina{\Sigma_\inp}
\newcommand\outa{\Sigma_\outp}
\newcommand\inout{{\inp\outp}}
\newcommand\inouta{\Sigma_\inout}

\newcommand{\expspace}{\textsc{Expspace}\xspace}

\def\stackrel#1#2{\mathrel{\mathop{#2}\limits^{#1}}}
% \newcommand{\intag}[1]{\stackrel{\inp}#1}
% \newcommand{\outtag}[1]{\stackrel{\outp}#1}

\newcommand{\intag}[1]{{#1}^\inp}
\newcommand{\outtag}[1]{{#1}^\outp}

% drat

\newcommand{\nat}{\mathbb{N}}
\newcommand{\Qin}{Q^{\inp}}
\newcommand{\Qout}{Q^{\outp}}
\newcommand{\Lin}{L^{\inp}}
\newcommand{\Lout}{L^{\outp}}
\newcommand{\Vin}{V^{\inp}}
\newcommand{\Vout}{V^{\outp}}
%\newcommand{\deltaout}{delta^{\outp}}
%\newcommand{\deltain}{delta^{\inp}}
\newcommand{\Sigmaend}{\Sigma_{\dashv}}
\newcommand{\seq}[1]{\bar{#1}}
\newcommand{\game}{\mathcal{G}}
\newcommand{\reduce}[1]{\inp(#1)}
\newcommand{\ST}{\mathcal{S}}
\newcommand{\pump}[2]{\mathit{pump}_{#1}(#2)}
\newcommand{\Pump}[2]{\mathit{Pump}_{\ge #1}(#2)}

\newcommand{\choice}[2]{\textsf{Ch}_{#1}^{#2}}
\newcommand{\prop}[1]{\textbf{\textsf{P}$_{#1}$}}
\newcommand{\propH}[1]{\textbf{\textsf{R}$_{#1}$}}
\newcommand{\outru}[1]{\textsf{out}_{#1}}
\newcommand{\outf}[1]{\textsf{fin}_{#1}}
\newcommand{\heap}[2]{\textsf{H}_{#1}^{#2}}
\newcommand{\heapf}[1]{\textsf{H}{(#1)}}


\newcommand{\oldbound}{N_{\tra}'}
\newcommand{\newbound}{N_{\tra}}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> On Equivalence and Uniformisation Problems for Finite Transducers/prelims.tex <==
\section{Automata and Transducers}\label{sec:prelims}


Let $\mathbb{N}$ denote the set of non-negative integers
$\{0,1,\dots\}$, and for every $n \in \mathbb{N}$, let $[n]$ denote the set $\{1,\ldots,n\}$.
Given a finite set $A$, let $|A|$ denote its cardinality.

 % of $A$ and let $\mathcal{P}(A)$ be set of subsets of $A$.
% Given two sets $A$ and $B$, let $\mathcal{F}(A,B)$ denote the set of
% functions from $A$ to $B$.

\vspace{1mm}
\noindent\textbf{Languages and Transductions of Words} An alphabet
$\Sigma$ is a finite set of symbols. The elements of the free monoid
$\Sigma^*$ are called \emph{words} over $\Sigma$. The length of a word $w$ is the number of its symbols. It is 
written $|w|$. The empty word (of length $0$) is denoted by $\epsilon$, and $\Sigma^+ = \Sigma^* \setminus\{\epsilon\}$ 
%For all $i\in\{1,\dots,|u|\}$, we denote by 
%$w[i]$ the $i$-th letter of $w$, and for all $j\in\{1,\dots,|u|\}$ such
%that $j\geq i$, by $w[i{:}j]$ the factor $w[i]w[i+1]\dots w[j]$. By
%$w[{:}i]$ (resp. $w[i{:}]$) we denote the prefix up to (and including)
%position $i$ (resp. the suffix from (and including) position $i$). We
%set $w[{:}0] =\epsilon$. 
%For $\Sigma'\subseteq \Sigma$, we define the morphism
%$\pi_{\Sigma'}$ from $\Sigma^*$ to $\Sigma'^*$ by
%$\pi_{\Sigma'}(\sigma) = \sigma$ if $\sigma\in \Sigma'$ and by
%$\pi_{\Sigma'}(\sigma) = \epsilon$ otherwise.
%For instance, if $\Sigma = \{a,b,c\}$ and $\Sigma' = \{a,b\}$, we have
%$\pi_{\Sigma'}(acbcb) = abb$ and $\pi_{\Sigma'}(ccc) = \epsilon$. 
The set $\Sigma^*$ can be partially ordered by the word prefix relation
$\preceq$.%, i.e., $u\preceq v$ if $u$ is a prefix of $v$. 



We denote by $\Sigma^{-1}$ the set of
symbols $\sigma^{-1}$ for all $\sigma\in\Sigma$. Any word $u\in
(\Sigma\cup \Sigma^{-1})^*$ can be reduced into a unique irreducible word $\overline{u}$ by the equations
$\sigma\sigma^{-1} = \sigma^{-1}\sigma = \epsilon$ for all
$\sigma\in\Sigma$. Let $G_\Sigma$ be the set of irreducible words over
$\Sigma\cup \Sigma^{-1}$. The set $G_\Sigma$ equipped with concatenation $u.v =
\overline{uv}$ is a group, called the free group over $\Sigma$. We denote by $u^{-1}$ the inverse
of $u$. E.g. $(a^{-1}bc)^{-1} = c^{-1}b^{-1}a$. For $u\in G_\Sigma$,
we denote by $|u|$ its number of symbols. E.g., $|a^{-1}b^{-1}| = 2$,
$|a^{-1}bc^{-1}| = 3$



 A \emph{language} $L$ over $\Sigma$ is a subset of
$\Sigma^*$. A \emph{transduction} $R$ over $\Sigma$ is a subset of 
$\Sigma^*\times \Sigma^*$. The \emph{domain} of $R$ is the set 
$\dom(R) = \{ u\ |\ \exists v\in\Sigma^*\cdot (u,v)\in R\}$. 
For a word $u\in\Sigma^*$, we denote by $R(u)$ the set $\{v\ |\
(u,v)\in R\}$, and extend this notation to languages $L$ by $R(L) =
\bigcup_{u\in L} R(u)$. When $R$ is a function, we simply write $R(u) = v$
instead of $R(u)=\{v\}$. Finally, we denote by $\id_{\Sigma^*}$ the
identity relation on $\Sigma^*$. 


% \vspace{1mm}
% \noindent \textbf{Relations with origin}
% Let $\Sigma$ be an alphabet.
% % Let $\origin{\Sigma}$ be the subset of $\Sigma^* \times \Sigma^* \times \mathcal{F}(\mathbb{N},\mathbb{N})$ composed of the elements $(v,w,f)$ such that the domain of $f$ is $[|w|]$ and its range is included in $\{0 \} \cup [|v|]$.
% The function $f$ can be thought of as a function mapping each letter of $w$ to a space between the letters of $v$.\\
% Let $\oporigin{\Sigma}$ be the subset of $\origin{\Sigma}$ composed of the elements $(v,w,f)$ such that $f$ is monotonous increasing.\\
% A (binary) relation with origin over $\Sigma^*$ is a subset of $\origin{\Sigma}$.
% It is called order preserving if it is a subset of $\oporigin{\Sigma}$.\\
% \\
% Consider the alphabet $\Sigma \times \{1,2\}$.
% There is a natural bijection between the languages over $\Sigma \times \{1,2\}$ and the order preserving relations with origin over $\Sigma^*$, that we shall now define mathematically.\\
% Let $\alpha = (\pi_1,\pi_2,f) : (\Sigma \times \{1,2\})^* \rightarrow \oporigin{\Sigma}$ be the bijection defined as follows.
% Given a word $w$ over the alphabet $\Sigma \times \{1,2\}$, there
% exists $n \in \mathbb{N}$, $a_1,\ldots,a_n \in \Sigma$ and
% $w_0,\ldots,w_n \in \Sigma^*$ such that $w =
% (w_0,2)(a_1,1)(w_1,2)\ldots(a_n,1)(w_n,2)$.

% Let $\pi_1(w) = a_1\ldots a_n$, let $\pi_2(w) = w_0\ldots w_n$ and let
% $f(w)$ be the monotonous increasing function mapping each $1 \leq i
% \leq |w_0 \ldots w_n|$ to the greatest $j$ such that $|w_0 \ldots w_j|
% \leq i$.

% Then $\alpha(w) = (a_1\ldots a_n, w_0\ldots w_n, f(w))$.\\
% Then, $R : \mathcal{L} \mapsto \bigcup_{w \in \mathcal{L}} \alpha(w)$
% is a bijection between the languages over $\Sigma \times \{1,2\}$ and
% the order preserving relations with origin over $\Sigma^*$.

\vspace{1mm}
\noindent\textbf{Automata} A (finite state) \emph{automaton} over a finite alphabet $\Sigma$ is a tuple $\aut  = (Q,I,F,\Delta)$, where
$Q$ is the finite set of states,
$I \subseteq Q$ is the set of initial states,
$F \subseteq Q$ is the set of final states,
and $\Delta \subseteq Q \times \Sigma^* \times Q$ is the finite transition relation.
Given a transition $(q,w,q') \in \Delta$, $q$ is called its source, $q'$ its target, and $w$ its label.
An automaton is called \emph{deterministic} if each of its transition
is labelled by a single letter, and it admits no pair of transitions
that have same source, same label, and different targets. 

A \emph{run} of $A$ on a word $u\in\Sigma^*$ from state $q$ to
state $p$ is either a single state $q\in Q$ if $u=\epsilon$ and $q=p$, or a word $r = (q_1,u_1,p_1)(q_2,u_2,p_2)\dots (q_n,u_n,p_n)\in\Delta^+$
if $u\in\Sigma^+$, where $u = u_1\dots u_n$, $q_1 = q$ and $p_n = p$, and for all
$i\in\{1,\dots,n-1\}$, $p_i = q_{i+1}$. We write
$q_1\xrightarrow{u}_A p_n$ (or simply $q_1\xrightarrow{u} p_n$) if
such a run exists.  A run $r$ from a state $q$ to a state $p$ is \emph{accepting} if
$q$ is initial and $p$ is final. The \emph{language} recognised by $\aut$, written $\lang{\aut}$, is
the set of words $w \in \Sigma^*$ such that there exists an accepting
run of $A$ on $w$. If $B$ is an automaton, we write $A\subseteq B$
(resp. $A\equiv B$) whenever $\lang{A}\subseteq
\lang{B}$ (resp. $\lang{A} = \lang{B}$). 

\vspace{1mm}
\noindent\textbf{Transducers}
A (finite state) \emph{transducer} over a finite alphabet $\Sigma$ is a tuple $\tra  = (Q,I,F,\Delta,f)$, where 
$Q$ is the finite set of states,
$I \subseteq Q$ the set of initial states,
$F \subseteq Q$ the set of final states,
$\Delta \subseteq Q \times \Sigma^* \times \Sigma^* \times Q$ the transition relation,
and $f : F {\rightarrow} \Sigma^*$ the final output function.


As for automata, a \emph{run} of a transducer is either a single state
or a sequence of transitions. The \emph{input}  (resp. \emph{output}) of a run $r =
(q_1,u_1,v_1,p_1)\dots (q_n,u_n,v_n,p_n)\in\Delta^*$ is $\inr(r) = u_1\dots u_n$
(resp. $\outr(r)=v_1\dots v_n$). If $r$ is reduced to a single state, its input
and output are both $\epsilon$. We say that $r$ is a run of $\tra$ on
$u_1\dots u_n$. We write $q\xrightarrow{u|v} p$ to
mean that there exists a run on input $u\in\Sigma^*$ whose output is
$v\in\Sigma^*$. In particular, $q\xrightarrow{\epsilon|\epsilon} q$
for all $q\in Q$. The notion of accepting run of automata carries over
to transducers. The \emph{transduction} recognised by $\tra$, written $\rel{\tra}$ is the set
of pairs $(u,vf(p)) \in \Sigma^* \times \Sigma^*$ such that there
exists an accepting run of $\tra$ on $u$ from a state $q$ to a state
$p$ whose output is $v$.  We define $\dom(\tra)$ as
$\dom(\rel{\tra})$. The class of \emph{rational transductions} is the class of relations definable by
finite state transducers. 


The \emph{input automaton} of $\tra$ is the automaton $\aut =
(Q,I,F,\Delta')$ over the alphabet $\Sigma$, where $\Delta' = \{
(q,u,q') | (q,u,v,q') \in \Delta \}$. A transducer is called \emph{real time} if each of its transition is labelled by a pair $(a,v)$, where $a \in \Sigma$ and $v \in \Sigma^*$.
A transducer is called \emph{sequential} if its input automaton is
deterministic\footnote{Our model of sequential transducers was originally called
  subsequential transducers in the literature. We follow the
  terminology of \cite{DBLP:journals/tcs/LombardyS06}, where it is discussed.}. Sequential transducers define \emph{sequential
  transductions}. 
A transducer is \emph{trim} if all its accessible
states are co-accessible, i.e. for all $q\in Q$, $q_0\in I$, $u,v\in\Sigma^*$,
if $q_0\xrightarrow{u\mid v}
q$, then there exist $u',v'\in\Sigma^*$ and $q_f\in F$ such that
$q\xrightarrow{u'\mid v'} q_f$. 

\vspace{2mm}
\noindent\textbf{Decision Problems for Transducers} Let $\tra_1,\tra_2$ be two transducers over an alphabet $\Sigma$. We
write $\tra_1\subseteq \tra_2$ whenever $\rel{\tra_1}\subseteq
\rel{\tra_2}$. The \emph{inclusion
problem} asks, given $\tra_1,\tra_2$, whether $\tra_1\subseteq
\tra_2$. Similarly, we define the equivalence problem by asking
whether $\rel{\tra_1} = \rel{\tra_2}$, denoted $\tra_1\equiv \tra_2$. 
Let $\tra$ be a transducer over an alphabet $\Sigma$.
A uniformiser of $\tra$ is a transducer $\uni$ such that
$\uni\subseteq \tra$ and $\dom(\uni) = \dom(\tra)$.
We sometimes write seq-uniformiser for sequential uniformiser. 
The \emph{sequential uniformisation problem} (seq-uniformisation
problem) asks, given a transducer $\tra$ over
$\Sigma$, whether $\tra$ admits a seq-uniformiser.

\begin{center}
\begin{figure}[t]
\vspace{-5mm}
\begin{center}
\subfloat[$\tra_1$]{
\begin{tikzpicture}[->,>=stealth',auto,node distance=3cm,thick,scale=0.7,every node/.style={scale=0.7}]
  \tikzstyle{every state}=[fill=yellow!30,text=black]
  % \tikzstyle{every edge}=[draw=black,text=red]
  \tikzstyle{initial}=[initial by arrow, initial where=left, initial text=]
  \tikzstyle{accepting}=[accepting by arrow, accepting where=right, accepting text=$\epsilon$]

  \node[initial,state] (A) at(0,0) {};
  \node[accepting,state] at(1.8,0) (B)  {};
  \path (A) edge node {$\begin{array}{l}\trans{a}{\epsilon}\end{array}$} (B);
  \path (A) edge [loop above] node {\trans{a}{aa}} (A);
  \path (B) edge [loop above] node {\trans{a}{\epsilon}} (B);
\end{tikzpicture}
}
\subfloat[$\tra_2$]{
\begin{tikzpicture}[->,>=stealth',auto,node distance=3cm,thick,scale=0.7,every node/.style={scale=0.7}]
  \tikzstyle{every state}=[fill=yellow!30,text=black]
  % \tikzstyle{every edge}=[draw=black,text=red]
  \tikzstyle{initial}=[initial by arrow, initial where=left, initial text=]
  \tikzstyle{accepting}=[accepting by arrow, accepting where=right, accepting text=$\epsilon$]

  \node[initial,state] (A) at(0,0) {};
  \node[accepting,state] at(1.8,0) (B)  {};
  \path (A) edge node {$\begin{array}{l}\trans{a}{\epsilon}\end{array}$} (B);
  \path (A) edge [loop above] node {\trans{a}{\epsilon}} (A);
  \path (B) edge [loop above] node {\trans{a}{aa}} (B);
\end{tikzpicture}
}%
\subfloat[$\tra$]{
\begin{tikzpicture}[->,>=stealth',auto,node distance=3cm,thick,scale=0.7,every node/.style={scale=0.7}]
  \tikzstyle{every state}=[fill=yellow!30,text=black]
  % \tikzstyle{every edge}=[draw=black,text=red]
  \tikzstyle{initial}=[initial by arrow, initial where=left, initial text=]
  \tikzstyle{accepting}=[accepting by arrow, accepting where=right, accepting text=$\epsilon$]

  \node[initial,state] (A) at(0,1) {};
  \node[initial,accepting,state] (B) at(1.8,1) {};
  \node[initial,state] (A2) at(0,-1) {};
  \node[state] (B2) at(1.8,-1) {};
  \node[accepting,state] (C2) at(3.6,-1) {};
  \path (B2) edge node {\trans{B}{\epsilon}} (C2);
  \path (A) edge node {\trans{A}{\epsilon}} (B);
  \path (A2) edge node {$\begin{array}{l}\trans{a}{\epsilon}\\ \trans{a}{a}\end{array}$} (B2);
  \path (A) edge [loop above] node {\trans{a}{a}} (A);
  \path (A2) edge [loop above] node {\trans{a}{\epsilon}} (A2);
  \path (B2) edge [loop above] node {\trans{a}{aa}} (B2);
\end{tikzpicture}
}
\subfloat[$U$]{
\begin{tikzpicture}[->,>=stealth',auto,node distance=3cm,thick,scale=0.7,every node/.style={scale=0.7}]
  \tikzstyle{every state}=[fill=yellow!30,text=black]
  % \tikzstyle{every edge}=[draw=black,text=red]
  \tikzstyle{initial}=[initial by arrow, initial where=left, initial text=]
  \tikzstyle{accepting}=[accepting by arrow, accepting where=right, accepting text=$\epsilon$]
  \tikzstyle{acceptingdown}=[accepting by arrow, accepting where=below, accepting text=$\epsilon$]

  \node[initial,acceptingdown,state] (A) at(0,1) {};
  \node[accepting,state] at(2,1) (B)  {};
  \path (A) edge node {\trans{A,B}{\epsilon}} (B);
  \path (A) edge [loop above] node {\trans{a}{a}} (A);
\end{tikzpicture}
}
\caption{Transducers such that $\tra_1\equiv \tra_2$ and $\tra$ is
  seq-uniformisable by $U$.}
\label{fig:notk} 
\vspace{-4mm}
\end{center}
\end{figure}
\end{center}

\vspace{-5mm}
\begin{example}\label{ex:trans}
    Consider the transducers $\tra_1$ and $\tra_2$ of
    Fig.~\ref{fig:notk} over the alphabet $\{a\}$. They both define
    the transduction $\{ (a^n, a^{2i})\mid n\geq 1,0 \le i \le n{-}1\}$
    and are therefore equivalent. The transducer $\tra$ is over the
    alphabet $\{a,A,B\}$ and defines the transduction $\{ (a^nA, a^n)\mid n\geq 0\}\cup \{ (a^nB, a^i)\mid
    n\geq 1,\ 0 \le i \le 2n{-}1\}$. It is uniformisable by the
    sequential transducer $U$ with $\rel{U} = \{ (a^n\alpha,
    a^n)\mid n\geq 0,\alpha\in\{A,B\}\}$. 
\end{example}




\begin{theorem}[\cite{DBLP:journals/jacm/Griffiths68,CarayolL14}]\label{thm:undecunif}
\hspace{-1mm}The inclusion, equivalence and sequential uniformisation problems for rational transductions are undecidable.
\end{theorem}

% For subclasses of transducers, decidability has been recovered. The
% largest known class with decidable inclusion and equivalence is the
% class of \emph{finite-valued transducers}
% \cite{GurIba83,CulKar86c,DBLP:conf/mfcs/Weber88,DBLP:conf/dlt/Souza08}, i.e. transducers $\tra$
% such that there exists $k\in\mathbb{N}$ and for all
% $u\in\dom(\rel{\tra})$, $|\rel{\tra}(u)|\leq k$. It is also known
% that any rational relation is effectively uniformisable by a rational
% function \cite{journals/iandc/Kobayashi69}.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> On Equivalence and Uniformisation Problems for Finite Transducers/rational.tex <==
\vspace{.5mm}
\noindent\textbf{Decision problems for transducers modulo rational
  resynchronisers} The $\mathbb{U}$-decision problems
are undecidable, this raises the question whether there is an interesting
class of resynchronisers for which we can recover decidability. 
It turns out that $\mathbb{U}$ is not rational. In
contrast, we show that, as long as $\sync$ is rational,
the $\sync$-decision problems are reducible to the
$\mathbb{I}$-decision problems, which in turn can be solved by reduction to
decidable problems of automata and two-player games. 


% % We shall begin by exposing the regular language inclusion problem, and the reduction from the $\mathbb{I}$-inclusion problem into it.


% % Given two automata $\aut_1$ and $\aut_2$, the inclusion problem asks whether $\lang{\aut_1}$ is included into $\lang{\aut_2}$.

% \begin{theorem}[reference needed]
% The regular language inclusion problem is decidable.
% \end{theorem}

\begin{restatable}{proposition}{decisionIproblems}\label{prop:Iinclusion}\label{prop:Iuniformisation}
The $\mathbb{I}$-inclusion and $\mathbb{I}$-equivalence problems are
\textsc{PSpace-complete}. The sequential $\mathbb{I}$-uniformisation problem is 
\textsc{ExpTime-complete}. 
\end{restatable}

\begin{proof}
First, note that $\tra_1\subseteq_{\mathbb{I}}\tra_2$ iff
$\lang{\tra_1}\subseteq \lang{\tra_2}$ iff $A_1\subseteq A_2$, where
$A_1,A_2$ are the underlying automata of $\tra_1,\tra_2$
respectively. Automata inclusion and equivalence problems are
\textsc{PSpace-complete}, and they easily reduce (by putting $\epsilon$
outputs) to $\mathbb{I}$-inclusion
and $\mathbb{I}$-equivalence.

To get \textsc{ExpTime} membership of seq-$\mathbb{I}$-uniformisation, for
a transducer $\tra$, we construct a two-player safety game $G_\tra =
(V = V_{\textsf{In}}\uplus V_{\textsf{Out}}, v_0, E)$ between an
adversary (Player \textsf{In}) who picks input symbols and controls
positions in $V_{\textsf{In}}$, and a protagonist
(Player \textsf{Out}) who picks sequences of output symbols and
controls positions in $V_{\textsf{Out}}$. Wlog we assume that $\tra$
has no final output function, by adding an endmarker $\dashv$ to words of
its domain. Let $\aut = (Q,q_0,F,\delta)$ be a complete DFA equivalent to the the underlying
automaton of $\tra$ (whose size is at most
exponential  in the size of $\tra$). Player positions have three
components: a residual language\footnote{A residual of a language $L$
  over some alphabet $\Sigma$ is a language $u^{-1}L = \{ v\mid uv\in L\}$ for $u\in \Sigma^*$.} of $\dom(\tra)$ that controls 
the possible continuations of the input word chosen so
far by  Player \textsf{In}, a state of $\aut$ and a round $r \in
\{\textsf{In},\textsf{Out}\}$. Let $\mathcal{D} = \{ u^{-1}\dom(\tra)\mid u\in\Sigma^*\}$
be the set of residuals of $\dom(\tra)$ (for example, represented by the states of 
the minimal DFA for $\dom(\tra)$, which can be computed in exponential time in the size of $\tra$). 
Then, $V_{\textsf{In}} = \mathcal{D}\times Q\times
\{\textsf{In}\}$ and $V_{\textsf{Out}} = \mathcal{D}\times Q\times
\{\textsf{Out}\}$. The initial position is $v_0  = (\dom(\tra), q_0,
\textsf{In})$ and the edge relation $E$ as follows: from a position 
$(D,q,\textsf{In})$, there are outgoing edges to all states
$(\sigma^{-1}D,\delta(q,\sigma^\inp), \textsf{Out})$ for all
$\sigma\in\Sigma$. From a position $(D,q,\textsf{Out})$, Player
$\textsf{Out}$ can pick any state $q'\in Q$ such that there exists a
sequence $v\in\outa^*$ such that $q\xrightarrow{v}_{\aut} q'$, and in
that case an outgoing edge to $(D, q', \textsf{In})$ is added to $E$. 
The \emph{unsafe positions} for Player \textsf{Out} are all positions
$(D,q,\textsf{In})$ such that $\epsilon\in D$ and $q\not\in F$: At
such positions, Player $\textsf{In}$ could choose to terminate the sequence
of input symbols (while staying in $\dom(T)$ since $\epsilon\in D$)
and the sequence of output symbols chosen by Player \textsf{Out},
mixed with the input symbols chosen by Player \textsf{In}, does not
belong to $L(\aut)$ (because $q\not\in F$). It can be shown that
Player \textsf{Out} has a strategy to avoid the unsafe positions in
$G_\tra$ iff there exists a seq-$\mathbb{I}$-uniformiser of $\tra$
(finiteness of the seq-$\mathbb{I}$-uniformiser comes from the fact that
safety games are memoryless determined). Since safety games can be solved in polynomial time and $G_\tra$ has exponential
size, we get the result. The results on safety games that we use here can be found, e.g., in \cite{GradelTW02}.

For the \textsc{ExpTime} lower bound, we note that in our formalism we
can model the synchronous uniformisation (or synthesis) problem, as
considered in \cite{PnuRos:89} for infinite words, by taking
synchronisations that strictly alternate between input and output. It
seems to be common knowledge in the synthesis community that the
synchronous uniformisation problem is \textsc{ExpTime-complete} if the
relation is given by a nondeterministic automaton. However, we were
not able to find a reference for this result. We thus give a reduction
from the acceptance problem for alternating \textsc{Pspace} Turing
machines in the appendix.
\end{proof}


For all transducers $\tra$ and synchronisers $\sync$,
$\sync(\lang{\tra})$ is a regular synchronisation language and by
Nivat's theorem (Theorem~\ref{thm:nivat}), there exists a transducer 
$\tra^\sync$ such that 
$\lang{\tra^\sync} = \sync(\lang{\tra})$. It implies that the
seq-$\sync$-uniformisation of $\tra$ reduces to the
seq-$\mathbb{I}$-uniformisation of $\tra^\sync$. Similar arguments apply
for inclusion and equivalence and, as a consequence of
Proposition~\ref{prop:Iuniformisation}, we obtain:


\begin{restatable}{theorem}{decisionSproblems}\label{thm:rat}
Let $\sync$ be a rational resynchroniser, given as a transducer.
The $\sync$-inclusion and $\sync$-equivalence problems are
\textsc{PSpace-complete}. The
sequential $\sync$-uniformisation problem is
\textsc{ExpTime-complete}. 
\end{restatable}


% We write $L_1\equiv L_2$ if $R(L_1) = R(L_2)$, and
% $L_1\subseteqq L_2$ if $R(L_1)\subseteq R(L_2)$. Given
% two binary relations $\triangle_1,\triangle_2$ over languages
% such that $\triangle_1 \subseteq\triangle_2$, we say that 
% $\triangle_1$ is finer than $\triangle_2$ and that
% $\triangle_2$ is coarser than $\triangle_1$. In this paper,
% we study language relations that are coarser than language
% equality (resp. inclusion) and finer than the transduction
% equivalence $\equiv$ (resp. the transduction inclusion
% $\subseteqq$). 


%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> On Equivalence and Uniformisation Problems for Finite Transducers/synch.tex <==
\section{Decision Problems Modulo Resynchronisers}\label{sec:synch}

A pair $(u,v)\in \Sigma^*\times \Sigma^*$ can be represented by a 
coloured word over $\Sigma\times \{\inp,\outp\}$,
where the colours indicate whether a symbol in $\Sigma$ is an input or an
output symbol. Such a coloured word is called a synchronisation of
$(u,v)$. 
More generally, any language over the alphabet $\Sigma\times \{\inp,\outp\}$ represents
s transduction $R\subseteq \Sigma^*\times \Sigma^*$, and is called a synchronisation language for $R$.
This way of representing transductions is analysed in \cite{conf/stacs/FigueiraL14}. 
What we call a resynchroniser below, is a transduction of synchronisations, that is, 
over words in $(\Sigma\times \{\inp,\outp\})^*$, that preserves
the represented pairs. In this section, we study stronger notion of
inclusion, equivalence and sequential uniformisation, parametrised by such a
resynchroniser. We show their decidability for rational resynchronisers
and introduce the class of bounded delay resynchronisers, and show that it
has appealing properties. 

\input synchronizers
\input decision
\input rational




%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> On Equivalence and Uniformisation Problems for Finite Transducers/synchronizers.tex <==


\vspace{1mm}
\noindent\textbf{Synchronisations and resynchronisers} 
Given an alphabet $\Sigma$, we let $\inouta = \Sigma\times
\{\inp,\outp\}$, $\ina = \Sigma\times
\{\inp\}$ and $\outa = \Sigma\times
\{\outp\}$. For $c\in \{\inp,\outp\}$, we write $\sigma^c$
instead of $(\sigma,c)$. The colouring $c$ can be seen as a morphism
$.^c : \Sigma^*\rightarrow \Sigma^*_c$ and we write $u^c$ its
application on a word $u\in\Sigma^*$. Conversely, for
$c\in\{\inp,\outp\}$, we define two
morphisms $\pi_c : \inouta^*\rightarrow \Sigma$ that extract the input
and output words, by $\pi_c(\sigma^c) = \sigma$ and $\pi_c(\sigma^d) =
\epsilon$, for all $\sigma\in\Sigma$, and $d\neq c$. %
% The \emph{input and output morphisms} of the words over $ (\inouta)^*$ are
% defined respectively as the monoid morphisms $\pi_\inp$ and
% $\pi_\outp$ generated by $\pi_\inp(\intag{\sigma}) = \sigma$,
% $\pi_\inp(\outtag{\sigma}) = \epsilon$, $\pi_\outp(\outtag{\sigma}) = \sigma$,
% $\pi_\outp(\outtag{\sigma}) = \epsilon$ for all $\sigma\in\Sigma$. 
Two words $u,v\in(\inouta)^*$ are said to be \emph{equivalent},
denoted by $u\sim_\inout v$, if 
$\pi_c(u)=\pi_c(v)$ for all $c\in\{\inp,\outp\}$.
For example, $a^\inp b^\inp a^\outp$ and $a^\inp a^\outp b^\inp$ are equivalent, and both are synchronisations of $(ab,a)$.  
Any language $L\subseteq \inouta^*$ defines a transduction
over $\Sigma$ defined by $\rel{L}\ =\ \{
(\pi_{\inp}(w),\pi_{\outp}(w))\in \Sigma^*\times \Sigma^*\mid w\in
L\}$, and $L$ is called a $\emph{synchronisation}$ of a transduction
$R\subseteq \Sigma^*\times \Sigma^*$ if $\rel{L} = R$. %
% Note that two different languages may define
% the same transduction. For instance, let $\Sigma = \{a,b\}$.
% Then $L_1 = \{ a^{\inp}b^{\outp} \}$ and $L_2 = \{
% b^{\outp}a^{\inp} \}$ are two different languages, but 
% $\rel{L_1} = \rel{L_2} = \{ (a,b)\}$. However if
% $L_1\subseteq L_2$, then $\rel{L_1}\subseteq \rel{L_2}$.
 % In this
% paper, we define several notions to compare languages $L_1,L_2$ such
% that $R(L_1) = R(L_2)$ or $R(L_1)\subseteq R(L_2)$. 
% \begin{proposition}
    % For all languages $L_1,L_2$ over $\inouta$, if $L_1\subseteq L_2$
    % then $\rel{L_1}\subseteq \rel{L_2}$.
% \end{proposition}
We also say that $L$
synchronises $R$. Note that two different languages may
synchronise the same transduction. 



Mapping a synchronisation to
another one is done through the notion of resynchroniser. A \emph{resynchroniser} is a transduction $\sync\subseteq
\inouta^*\times \inouta^*$, such that $(i)$
$\id_{\inouta^*}\subseteq \sync$ and $(ii)$ for all
$(w,w')\in\sync$, it holds $w\sim_\inout w'$.
For instance, the identity relation $\id_{(\inouta)^*}$ is a
resynchroniser that we shall denote by $\mathbb{I}$, as well as the relation $\mathbb{U}_{\inouta}  = \{
(w,w')\in \inouta\mid w\sim_\inout w'\}$, called the \emph{universal resynchroniser} 
over $\inouta$. We write $\mathbb{U}$ instead of
$\mathbb{U}_{\inouta}$ when it is clear from the context.
Note that for any resynchroniser $\sync$, we have
$\id_{\inouta^*}\subseteq \sync \subseteq \mathbb{U}$. %
% Observe that condition $(1)$ implies that $\dom(\sync) =
 % (\inouta)^*$ and $L\subseteq \sync(L)$.
% Note that there is in general infinitely many synchronisations for a
% transduction.
The properties $(i)$ and $(ii)$ of resynchronisers are chosen such that
they preserve the represented transductions, as stated in the proposition below.
% \begin{proposition}
% Let $L$ be a synchronisation for a transduction $R$ and $\sync$ a
% resynchroniser. Then $\sync(L)$ synchronises $R$, i.e. $R = \rel{L} =
% \rel{\sync(L)}$.
% \end{proposition}
\begin{proposition}
For all $L\subseteq \inouta^*$ and all resynchronisers $\sync\subseteq
\inouta^*\times \inouta^*$, $\rel{L} = \rel{\sync(L)}$.
\end{proposition}
Classes of synchronisation languages and their correspondence with the classes of rational
relations they synchronise have been studied in \cite{conf/stacs/FigueiraL14}. 
We can formulate in this framework a result known as Nivat's
theorem \cite{Niv-transductions-lc} as follows.
\begin{theorem}{\cite{Niv-transductions-lc}}\label{thm:nivat}
    A transduction $R$ is rational iff it is synchronised by a regular language.
\end{theorem}
 
Any transducer $\tra  = (Q,I,F,\Delta,f)$ naturally defines a regular
synchronisation for $\rel{\tra}$ by its \emph{underlying automaton}, which is
the automaton obtained by concatenating the pairs of input and output words 
on the transitions and marking them with the respective symbol from $\{\inp,\outp\}$.
Formally, it is the 
automaton $A = (Q \cup \{ q_\dashv\},I, \{ q_\dashv\}, \Delta')$ over
$\inouta$, where $\Delta' = \{(q,v^{\inp}w^{\outp},q') | (q,v,w,q')
\in \Delta \} \cup \{(q,f(q)^{\outp},q_\dashv)|q \in F \}$. The \emph{language recognised by $\tra$} is the language 
recognised by its underlying automaton, denoted by $\mathcal{L}_{\tra}$, i.e. $\lang{\tra} =
\lang{A}$. Obviously, $\lang{\tra}$ is a synchronisation for the
relation $\rel{\tra}$, i.e. $\rel{\lang{\tra}} = \rel{\tra}$. 


%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> drat-uniformizer-to-strategy.tex <==
\newcommand{\pump}[2]{\mathit{pump}_{#1}(#2)}
\newcommand{\Pump}[2]{\mathit{Pump}_{\ge #1}(#2)}

We prove the existence of a winning strategy for Output in case that $R_\tra$
is uniformized by a sequential transducer. A note for the reader who
is not very familiar with this kind of game-theoretic reasoning: The
strategy that we construct below is not positional, it uses a memory of unbounded size. Furthermore, we do not even need to care whether we can compute the individual moves. Proving the existence of some strategy is sufficient and implies the existence of a positional strategy, as assumed in the proof of Lemma~\ref{lem:drat-strategy-to-uniformizer}.

\begin{lemma}\label{lem:drat-uniformizer-to-strategy}
  If $R_\tra$
  can be uniformized by a sequential transducer, then Output has a
  winning strategy in $\game_\tra$.
\end{lemma}



The rest of this section is devoted to the proof of Lemma~\ref{lem:drat-uniformizer-to-strategy}, which requires some definitions and other lemmas. For the construction of the strategy, we split the transformation sequence in a game position in two parts, both of length at most $K$. So we consider game positions of the form $(p,\rho\xi,d)$ with $|\rho| \le K+1$ and $|\xi| \le K$. The moves of type (Out3), which apply the operation $\reduce{\cdot}$ to an infix of the transformation sequence, are only applied to the second part $\xi$ of the transformation sequence. The first part $\rho$ remains fixed until it is consumed by an output move of type (Out2). 

Input word $u$ that generates the part $\xi$ of the transformation sequence is stored in the memory of the strategy, together with the information to which parts the operation $\reduce{\cdot}$ was applied (the operation $\reduce{\cdot}$ is applied to parts of the transformation sequence, but each such part corresponds to a part of $u$).
This leads to a structure of the form $(u,M)$ with a set $M$ of edges $(i,j)$, where $i < j$ are positions in $u$. These edges are well-nested (they do not cross). In the construction of the strategy, we need to refer to words that are obtained from $u$ by pumping the parts of $u$ enclosed by an edge.  Hence, we refer to $(u,M)$ as a \emph{pump-word}. 

Formally, pump-words $(u,M)$ and their corresponding transformation sequences $\rho_{(u,M)}$ are defined inductively as detailed below. 
Along the inductive definition we also define how to concatenate two pump-words.

%For these pumping operations we require that the edges $(i,j)$ are such that the infix $u[i,j]$ of $u$, and the infix of $\xi$ corresponding to $u[i,j]$ are idempotent and absorbed. This ensures that pumping the infixes corresponding to the edges does not change the profile of the word.
%
%Before we give the precise conditions that pump-words $(u,M)$ have to satisfy, we  define 

\begin{definition}\label{def:pump-word}
\begin{enumerate}
\item For each $u \in \Sigmaend^*$, $(u,\emptyset)$ is a pump-word. The transformation sequence of $(u,\emptyset)$ is $\rho_{(u,\emptyset)} := \rho_u$, the transformation sequence induced by $u$.
\item The concatenation of two pump-words $(u_1,M_1)$ and $(u_2,M_2)$ is defined in the expected way as $(u_1,M_1)(u_2,M_2) = (u_1u_2,M_1 \cup (M_2 + |u_1|))$, where $M_2 + |u_1|$ denotes the set of edges in $M_2$ shifted by $|u_1|$ to the right. For example $(aba,\{(1,2)\})(bbc,\{(1,3)\}) = (ababbc,\{(1,2),(4,6)\}$. 

%If $(u,M) = (u_1,M_1)(u_2,M_2)$, then the transformaiton sequence is defined as $\rho_{(u,M)} = \rho_{(u_1,M_1)} \circ  \rho_{(u_2,M_2)}$.

\item Let $(u,M)$ be a pump-word and let $\xi = \rho_{(u,M)}$ to simplify notation. Let $\xi = \xi_1\xi_2\xi_3$, where $\xi_1,\xi_2,\xi_3$ are transformation sequences and $|\xi_2| \ge 2$. Let $(u,M) = (u_1,M_1)(u_2,M_2)(u_3,M_3)$ be the corresponding split of $(u,M)$, that is, $\rho_{(u_i,M_i)} = \xi_i$ for all $i \in \{1,2,3\}$. 
If $P_{x_2}$ is idempotent and $P_{u_2}$ is idempotent, then $(u,M') = (u_1,M_1)(u_2,M_2 \cup \{(1,|u_2|)\})(u_3,M_3)$ is a pump-word, and $\rho_{(u,M')} := \xi_1\reduce{\xi_2}\xi_3$ is the transformation sequence of $(u,M')$.

Note that $M' = M \cup \{(|u_1|+1,|u_1|+|u_2|)\})$ according to the definition of concatenation of pump-words. \qed
\end{enumerate}
\end{definition}
In point~3 of Definition~\ref{def:pump-word}, we implicitly assume that the split $(u,M)) = (u_1,M_1)(u_2,M_2)(u_3,M_3)$ that is induced by the split $\xi = \xi_1\xi_2\xi_3$ does not ``cut'' any edge of $M$ (all edges of $u$ are inside $u_1$, $u_2$, or $u_3$). This follows from the fact that an infix $v$ of $u$ that is enclosed by an edge only contributes a single transformation $\reduce{\rho_v}$ to  $\rho_{(u,M)}$.

%Point 2 is only needed to define the concatenation of pump-words, which is used in point 3. 

As mentioned earlier, the edges in a pump-word mark factors that we want to pump. In the following, when we speak of a pumping factor, then we refer to an infix of $u$ that corresponds to an edge. For a pump-word $(u,M)$ and a number $k$, we define the set $\Pump{k}{(u,M)}$, which is obtained by repeating each pumping factor at least $k$ times:

\begin{itemize}
\item If $M = \emptyset$, then $\Pump{k}{(u,M)} = \{u\}$.
%\item If $(u,M) = (u_1,M_1)(u_2,M_2)$, then $\pump{k}{(u,M)} = \pump{k}{(u_1,M_1)}\pump{k}{(u_2,M_2)}$ and $\Pump{k}{(u,M)} = \Pump{k}{(u_1,M_1)}\Pump{k}{(u_2,M_2)}$.
\item If $(u,M) = (u_1,M_1)(u_2,M_2 \cup \{(1,|u_2|)\})(u_3,M_3)$ as in point 3 of Definition~\ref{def:pump-word}, then
 $\Pump{k}{(u,M)} = \bigcup_{\ell \ge k} \Pump{k}{(u_1,M_1)}(\Pump{k}{(u_2,M_2)})^\ell\Pump{k}{(u_3,M_3)}$ 
\end{itemize}
Clearly, $\Pump{k}{(u,M)}$ is a regular set for each $k$ and each $(u,M)$.

The condition on the profiles of pumping factors being idempotent, ensures that pumpings do not change profiles, as expressed in the following lemma.
\begin{lemma} \label{lem:pump-word-profile}
If $(u,M)$ is a pump-word, then $P_w = P_u$ for each word $w \in \Pump{1}{(u,M)}$.  
\end{lemma}
\begin{proof}
  The proof is by induction on the complexity of $(u,M)$, which is a mapping $\varphi: \nat \rightarrow \nat$ where $\varphi(n)$ is the number of edges in $M$ that are of nesting depth $n$. The nesting depth of an edge $(i,j)$ is defined as $1$ if there are no other edges inside $(i,j)$, and otherwise it is $n+1$ if the maximal nesting depth of an edge inside $(i,j)$ is $n$.
Note that $\varphi(n) > 0$ for only finitely many $n$.

We use the a lexicographic ordering for comparing these mappings, letting $\varphi_1 < \varphi_2$ if $\varphi_1(n) < \varphi_2(n)$ for the biggest $n$ with $\varphi_1(n) \not= \varphi_2(n)$ (note that such an $n$ exists if $\varphi_1 \not= \varphi_2$, as there are only finitely many non-zero entries). This is a well-ordering \cite{Dickson13} and thus can be used for an induction.

For the induction base, if $\varphi$ maps everything to $0$, then $M = \emptyset$ and $w = u$. 

So consider the last edge that has been added to $M$ according to Definition~\ref{def:pump-word}. This means that $(u,M) = (u_1,M_1)(u_2,M_2 \cup \{1,|u_2|\})(u_3,M_3)$, where the edge enclosing $u_2$ is the last one that was added. Then $w = w_1w_{2,1}\cdots w_{2,\ell}w_3$ with $w_1 \in \Pump{k}{(u_1,M_1)}$, $w_{2,1},\cdots, w_{2,\ell} \in \Pump{k}{(u_2,M_2)}$, and $w_3 \in \Pump{k}{(u_3,M_3)}$. Note that $(u_1,M_1)(u_2,M_2)^\ell(u_3,M_3)$ is a pump-word, and its complexity is smaller than the one of $(u,M)$ because the edge enclosing $u_2$ is removed and the iteration of $(u_2,M_2)$ only increases the number of edges of smaller nesting depth.

Then by induction, $P_{w_1w_{2,1}\cdots w_{2,\ell}w_3} = P_{u_1(u_2)^\ell u_3}$, and since $P_{u_2}$ is idempotent, we obtain $P_{u_1(u_2)^\ell u_3} = P_{u_1u_2u_3} = P_u$ for $\ell \ge 1$.
\end{proof}


The pump-words that we build during the strategy construction apply point 3 of Definition~\ref{def:pump-word} to saturation witnesses (see Section~\ref{subsec:profiles-and-saturated-sequences}). So they satisfy some further properties that, intuitively, ensure that outputs matching pumped words can be replaced by outputs matching the unpumped words. We refer to such pump-words as \emph{safe}:
 
\begin{definition}\label{def:safe-pump-word}
A pump-word is called \emph{safe} if in Definition~\ref{def:pump-word}(3) the following additional conditions are satisfied (using the same notations as in Definition~\ref{def:pump-word}(3)): 
\begin{itemize}
\item $M_3 = \emptyset$, so there are no edges after the one that is newly introduced.
\item $P_{\xi_1} = P_{\xi_1}P_{\xi_2}$ ($\xi_2$ is absorbed by $\xi_1$).
\item $P_{u_1} = P_{u_1}P_{u_2}$ ($u_2$ is absorbed by $u_1$).
\end{itemize}
The connection of saturation witnesses (see Section~\ref{subsec:profiles-and-saturated-sequences}) and the condition for safe pump-words is as follows. Let $\xi = \tau_1 \cdots \tau_{|\xi|}$, and  let $(u,M) = (u_1',M_1') \cdots (u_{|\xi|}',M_{|\xi|}')$ be the corresponding split of $(u,M)$ (that is, $\rho_{(u_i',M_i')} = \tau_i$). Let $\bar{P} = P_{u_1},\cdots, P_{u_{|\xi|}}$. Then the conditions for safe pump-words implies that $\xi_1\xi_2\xi_3$ is a saturation witness for $\xi$ and $\bar{P}$. Since $(u,M)$ determines $\xi = \rho_{(u,M)}$, and $\bar{P}$, we call this a \emph{saturation witness for $(u,M)$}. \qed
\end{definition}
The reason for considering pump-words and safe pump-words (and not just defining the latter) is that in a decomposition of a safe pump-word $(u,M) = (u_1,M_1)(u_2,M_2)(u_3,M_3)$, the part $(u_2,M_2)$ needs not to be safe (the condition of safe pump-word refers to the prefixes before the pumping factors). However, $(u_2,M_2)$ is a pump-word because being idempotent is a local property that does not depend on the prefix. 


The following lemma is essential for the strategy construction. It basically states that if an output word that matches a large pumping of $(u,M)$, then there is also an output word matching $\rho_{(u,M)}$, that is, an output that is consumed outside the pumping factors of $(u,M)$.
\begin{lemma} \label{lem:output-large-pumping}
  Let $(u,M)$ be a safe pump-word, $p,q \in Q$, and $v \in \Sigmaend^*$ be an output word such that there is $w \in \Pump{3|v|}{(u,M)}$ with $v \in \Lout(p,\rho_w,q)$. Then $\Lout(p,\rho_{(u,M)},q) \not= \emptyset$.
\end{lemma}
\begin{proof}
  The proof is by induction on the complexity of $(u,M)$, as in the proof of Lemma~\ref{lem:pump-word-profile}. If $M = \emptyset$, and the claim obviously holds because $w = u$ (there are no pumping factors) and $\rho_u = \rho_{(u,\emptyset)}$.

So consider the last edge that has been added to $M$ according to Definition~\ref{def:safe-pump-word}. This means that $(u,M) = (u_1,M_1)(u_2,M_2 \cup \{1,|u_2|\})(u_3,M_3)$, where the edge enclosing $u_2$ is the last one that was added. And as in the definition of pump-words, let $\xi_i = \rho_{(u_i,M_i)}$. We want to show that $\Lout(p,\xi_1\reduce{\xi_2}\xi_3,q) \not = \emptyset$.

By definition of $\Pump{3|v|}{(u,M)}$, we can write $w = w_1 w_{2,1}\cdots w_{2,\ell} w_3$ with $\ell \ge 3|v|$, $w_1 \in \Pump{3|v|}{(u_1,M_1)}$, $w_3 \in \Pump{3|v|}{(u_3,M_3)}$, and $w_{2,i} \in \Pump{3|v|}{(u_2,M_2)}$. Note that $P_{w_1} = P_{u_1}$, $P_{w_{2,i}} = P_{u_2}$, and $P_{w_3} = P_{u_3}$ by Lemma~\ref{lem:pump-word-profile}.

According to the definition of $\Lout(p,\rho_w,q)$, we can write $v = v_1v_{2,1}\cdots  v_{2,\ell} v_3$ with $v_1 \in \Lout(p,\rho_{w_1},q_2^0)$, each $v_{2,i} \in \Lout(q_2^{i-1},\rho_{w_{2,i}},q_2^i)$, and $v_3 \in \Lout(q_2^\ell,\rho_{w_3},q)$ for some states $q_2^0, \ldots, q_2^\ell$.

Since $\ell \ge 3|v|$, there must be an $i < 2|v|$ with $v_{2,i} = v_{2,{i+1}} = \varepsilon$. By definition of profiles we obtain $(q_2^{i-1},\varepsilon, q_2^i) \in P_{u_2}$ and $(q_2^i,\varepsilon, q_2^{i+1}) \in P_{u_2}$.  Since $P_{u_2}$ is idempotent by definition of pump-words, we obtain $(q_2^{i-1},\varepsilon, q_2^{i+1}) \in P_{u_2}$, and thus $q_2^i = q_2^{i+1}$ (see Lemma~\ref{lem:profile-properties}). We conclude that $(q_2^i, \varepsilon, q_2^i) \in P_{u_2}$, and $q_2^j = q_2^i$ and $v_{2,j} = \varepsilon$ for each $i \le j \le \ell$. 

Let $q_2 := q_2^i$, $w' =  w_1w_{2,1} \cdots w_{2,{2|v|}}$ and $v' = v_1v_{2,1} \cdots v_{2,{2|v|}}$. As a consequence of the above considerations, $v' \in \Lout(p,\rho_{w'},q_2)$.
Note that $(u_1,M_1)(u_2,M_2)^{2|v|}$ is a safe pump-word of smaller complexity than the one of $(u,M)$ (the edge enclosing $u_2$ in $(u,M)$ was removed, and the iteration of $(u_2,M_2)$ only adds edges of smaller nesting depth). Furthermore $w' \in \Pump{3|v|}{(u_1,M_1)(u_2,M_2)^{2|v|}}$, and $3|v| \ge 3|v'|$. We can thus apply the induction and obtain that $\Lout(p,\xi_1(\xi_2)^{2|v|},q_2) \not= \emptyset$. Since  $P_{\xi_2} = P_{\xi_2}P_{\xi_2}$ and $P_{\xi_1} = P_{\xi_1}P_{\xi_2}$, we conclude that $\Lout(p,\xi_1,q_2) \not= \emptyset$. 

From $(q_2,\varepsilon,q_2) \in P_{u_2}$ (as deduced above), we obtain $\varepsilon \in \Lout(q_2,\rho_{u_2},q_2)$, which implies $\varepsilon \in \Lout(q_2,\reduce{\rho_{u_2}},q_2)$ (see Lemma~\ref{lem:empty-word-traversal}). Since $\reduce{\rho_{u_2}} = \reduce{\rho_{(u_2,M_2)}} = \reduce{\xi_2}$, we conclude that $\Lout(q_2,\reduce{\xi_2},q_2) \not= \emptyset$.

Finally, note that $M_3 = \emptyset$ in the definition of safe pump-word. Hence $w_3 = u_3$, and $\xi_3 = \rho_{u_3}$. Thus $v_3 \in \Lout(q_2^\ell,\xi_3,q)$ because $P_{w_3} = P_{u_3}$.

Putting all these together, we obtain that $\emptyset \not= \Lout(p,\xi_1,q_2)\Lout(q_2,\reduce{\xi_2},q_2)\Lout(q_2,\xi_3,q) \subseteq \Lout(p,\xi_1\reduce{\xi_2}\xi_3)$ as desired. 
\end{proof}


\subsubsection*{An invariant for the strategy}

Before we start the construction of the strategy, we introduce one more terminology concerning uniformizers that  simplifies the presentation below. Recall the definition of the relation $R_p^\rho$ from Section~\ref{subsec:langauges-and-relations-of-transformation-sequences}. Every output in this relation has to start with a prefix in $\Lout(p,\rho)$. We say that a sequential uniformizer $S$ of $R_p^\rho$ is a \emph{$(p,\rho)$-uniformizer} if 
\begin{itemize}
\item in every run, the first non-empty output that $S$ produces has a prefix in $\Lout(p,\rho)$, and
\item $S$ outputs the endmarker only if it reads the endmarker on the input.
\end{itemize}
So with $(p,\rho)$-uniformizers we exclude the case that the prefix from $\Lout(p,\rho)$ is built up incrementally along several transitions, and the case that an endmarker is produced on the output before the endmarker has appeared on the input. It is quite easy to see that working with $(p,\rho)$-uniformizers is not a restriction.

\begin{remark}
If there is a sequential uniformizer for $R_p^\rho$, then there is also a $(p,\rho)$-uniformizer. 
\end{remark}
\begin{proof}
First note that for each $q \in Q$ the language $\Lout(p,\rho,q)$ is regular. 
Given a sequential uniformizer $S$ for $R_p^\rho$, one can construct a $(p,\rho)$-uniformizer $S'$ as follows. It mimics the transitions of $S$ but instead of producing output, it simulates 
DFAs for each $\Lout(p,\rho,q)$ on the output that $S$ would have produced. If the DFA for $\Lout(p,\rho,q)$ reaches an accepting state, then $S'$ produces some output word in $\Lout(p,\rho,q)$, appending the possibly remaining part $v$ of the output from the last transition. 

The property concerning the endmarker is easily achieved by delaying the output of it to the transition that reads $\dashv$ on the input.
\end{proof}

%A memory state of the strategy $f_\tra$ that we construct from $\tra$ is of the form $[(d,p,\rho,\xi),(u,M)]$ where  $(d,p,\rho\xi)$ is the current vertex of the play, $|\rho|,|\xi|\le K$, and $(u,M)$ is a pump-word with $\rho_{(u,M)} = \xi$. 
We construct a strategy $f_\tra$ from $\tra$, such that an invariant is maintained in each move, from which follows that $f_T$ is winning. The invariant is stated below. Condition (Inv0) only describes some properties on the structure of the memory that is used for $f_\tra$. Condition (Inv1) implies that $f_\tra$ is a winning strategy. The conditions (Inv2) and (Inv3) state intuitively that it is still possible to uniformize the remaining relation w.r.t.\ the input and output moves that have already been played.

For a sequential transducer $S$ and an input word $w$, we write $S(w)=v$ if $S$ produces output $v$ when reading input $w$.

\begin{itemize}
\item[(Inv0)] The memory states of $f_\tra$ are of the form $[(p,\rho,d',\xi,d),(u,M)]$, where 
  \begin{enumerate}[(i)]
  \item the current game position is of the form $(p,\rho\xi,d)$ or $(p,\rho\xi,d,a)$ (the memory maintains two parts of the transformation sequence in the game position;  $f_\tra$ only applies moves of type (Out3) to the second part $\xi$);
  \item  $|\rho| \le K+1$, $|\xi| \le K$;
  \item $(u,M)$ is a safe pump-word with $\rho_{(u,M)} = \xi$ ($u$ is the input sequence that induced $\xi$, and $M$ corresponds to the applications of moves of type (Out3));
  \item if $\xi$ is saturated, then a saturation witness for $(u,M)$ is of the form $\xi_1\xi_2\xi_3$ with $\xi_3 = \varepsilon$ (new edges to $u$ will be added only at the end of the word);
  \item $A_\dom: d' \xrightarrow{u} d$ (before reading $u$, the automaton $A_\dom$ was in state $d'$). 
  \end{enumerate}
\item[(Inv1)] If $d \in F_\dom$, then $\rho = \xi = \varepsilon$ and $p \in F$.
\item[(Inv2)] If $d \notin F_\dom$, then there is a $(p,\rho)$-uniformizer, and the domain of $R_p^{\rho}$ contains all words from $L(A_\dom,d')$, which is the set of word accepted by  $A_\dom$ from state $d'$. 
\item[(Inv3)] For every $(p,\rho)$-uniformizer $S$ there is $w \in \Pump{|S|!}{(u,M)}$ such that $S(w) = \varepsilon$.
\end{itemize}

The last condition (Inv3) is used to build a $(q,\xi)$-uniformizer (ensuring (Inv2) in the new vertex), once the strategy is ready to play an output in $\Lout(p,\rho,q)$ that consumes $\rho$ from the lookahead. The choice of $|S|!$ for the number repetitions in the pumping ensures that $S$ enters a loop on each of the pumped factors. This is useful in the proofs below. 


\begin{lemma} \label{lem:invariant-implies-winning}
  If the strategy $f_\tra$ satisfies the properties (Inv0)--(Inv3), then it is a winning strategy. 
\end{lemma}
\begin{proof}
This is a direct consequence of  (Inv1).
\end{proof}


The next lemma is the key lemma for preserving the invariant in a move that produces output. It covers the case that (Inv3) fails after appending the next input letter $a$. Then the goal is to produce output that consumes $\rho$ and to transfer the property (Inv2) to $\xi \circ \tau_a$.
\begin{lemma} \label{lem:propagate-invariant}
Let $[(p,\rho,d',\xi,d),(u,M)]$ be a memory state that satisfies (Inv0)--(Inv3). Let $a \in \Sigmaend$ be such that $S(wa) \not= \varepsilon$ for all $w \in \Pump{|S|!}{(u,M)}$ for some $(p,\rho)$-uniformizer $S$. Then there exists $q \in Q$ such that 
\begin{itemize}
\item $\Lout(p,\rho,q) \not= \emptyset$, 
\item The domain of $R_q^{\xi \circ \tau_a}$ contains all words in $L(A_\dom,d_a)$ with $d_a = \delta_\dom(d,a)$, 
\item and if $a \not= \dashv$, there is a $(q,\xi \circ \tau_a)$-uniformizer.  
\end{itemize}
\end{lemma}
\begin{proof}
By (Inv3), there is  $w \in \Pump{|S|!}{(u,M)}$ such that $S(w) = \varepsilon$. Let $s_0$ be the initial sate of $S$, and $s',s$ be the states of $S$ such that $S: s_0 \xrightarrow{w/\varepsilon} s' \xrightarrow{a/yz} s$, where $y \in \Lout(p,\rho,q)$ for some state $q$ (the first non-empty output contains a prefix in $\Lout(p,\rho)$). This proves the existence of $q \in Q$ such that $\Lout(p,\rho,q) \not= \emptyset$.

Since $S$ does not see the difference between a factor repeated $\ell \ge |S|!$ times or $\ell + k|S|!$ times, one can even find $w_k \in  \Pump{k|S|!}{(u,M)}$ for each $k\ge 1$ such that $S(w_k) = \varepsilon$ and furthermore, $S$ reaches the same state $s'$ after reading $w_k$ for all $k$. So $S: s_0 \xrightarrow{w_k/\varepsilon} s' \xrightarrow{a/yz} s$ for all $k$ 

Let $x \in L(A_\dom,d_a)$. Then $uax \in L(A_\dom,d')$ because:
\[
  A_\dom: d' \xrightarrow{u} d \xrightarrow{a} d_a \xrightarrow{x} F_\dom.
\]
Since the pumped words of $(u,M)$ induce the same state transformation on $A_\dom$ as $u$, we obtain that $w_kax \in L(A_\dom,d')$ for all $k$.
Let $z_x$ be the output produced by $S$ on input $x$ from state $s$. Then
\[
S: s_0 \xrightarrow{w_k/\varepsilon} s' \xrightarrow{a/yz} s \xrightarrow{x/z_x} F_S
\]
for each $k$, where $F_S$ is the set of final states of $S$.
This implies that $\delta^*(q,w_kax,zz_x) = (r_k,\varepsilon,\varepsilon)$ with $r_k \in F$ for each $k$ because $S$ is a $(p,\rho)$-uniformizer. So for each $k$, $zz_x$ has a prefix $v_k$ such that $\delta^*(q,w_ka,v_k) = \delta^*(q_k',a,\varepsilon) = (q_k,\varepsilon,\varepsilon)$ for some state $q_k$. In other words, $v_k \in \Lout(q,\rho_{w_ka},q_k)$.

Since there are only finitely many possible prefixes $v_k$ and states $q_k$,  there are infinitely many $k$ with the same $v_k$ and the same $q_k$. By choosing the corresponding subsequence of $w_1,w_2,\ldots$, we can assume that all $v_k$ and $q_k$ are the same, so we just denote them by $v_1$ and $q_1$.

We obtain that $v_1 \in \Lout(q,\rho_{w_ka},q_1)$ for all $k$. By choosing $k = 3|v_1|$, we can apply Lemma~\ref{lem:output-large-pumping}, and obtain that $\Lout(q,\xi \circ \tau_a,q_1) \not= \emptyset$. 

We can conclude that  $x \in \dom(R_q^{\xi \circ \tau_a})$ as follows. The output word $zz_x$ was shown to be the form $v_1v'$. We can replace the prefix $v_1$ by some word $v'' \in \Lout(q,\xi \circ \tau_a,q_1)$. Then $(x,v''v') \in R_q^{\xi \circ \tau_a}$.

It remains to prove that there is a $(q,\xi \circ \tau_a)$-uniformizer $S'$ in case $a \not= \dashv$. The reason for excluding $\dashv$ is that in this case there are no further transitions of $S$ from $s$.

We already proved that for each input $x \in L(A_\dom,d_a)$, the output word $zz_x$ (as above) is of the form $v_1v'$ with $v_1 \in \Lout(q,\rho_{w'a},q_1)$ for some $w' \in  \Pump{|S|!}{(u,M)}$ with $S:s_0 \xrightarrow{w'/\varepsilon} s'$, and some state $q_1$, such that $\Lout(q,\xi \circ \tau_a,q_1) \not= \emptyset$. And then $(x,v''v') \in R_q^{\xi \circ \tau_a}$ for $v'' \in \Lout(q,\xi \circ \tau_a,q_1)$.

The idea for constructing a $(q,\xi \circ \tau_a)$-uniformizer $S'$ is that we modify $S$ to detect a prefix of the output with the properties of $v_1$ as above, and then replace it by $v''$. To implement this operation, we show that the set of output strings $v_1$ with the above property is regular, by using the following observations:
\begin{itemize}
\item $L_1 := \Pump{|S|!}{(u,M)}$ is regular.
\item $L_2 := \{w' \in \Sigmaend^* \mid S:s_0 \xrightarrow{w'/\varepsilon} s'\}$ is regular.
\item For each $q_1$, the set $L_{q_1}$ of output strings $v_1$ such that there exists $w' \in L_1 \cap L_2$ and $v_1 \in \Lout(q,\rho_{w'a},q_1)$ is regular. An automaton for this set reads $v_1$, guesses $w'$, simulates $\tra$ from $q$ on the pair $(w',v_1)$, and simulates an automaton for $L_1 \cap L_2$ on the guessed $w'$. 
\end{itemize}
So the $(q,\xi \circ \tau_a)$-uniformizer $S'$ simulates  the transitions of $S$ starting from state $s$, and in parallel simulates for each $q_1 \in Q$ such that $\Lout(q,\xi \circ \tau_a,q_1) \not= \emptyset$ an automaton for $L_{q_1}$ on $z$ followed by the output produced in the simulation of $S$. During this simulation, $S'$ does not produce any output. As observed earlier, for some $q_1$,  the automaton for $L_{q_1}$ will eventually reach an accepting state. In this transition, $S'$ produces an output string $v''$ in $\Lout(q,\xi \circ \tau_a,q_1)$ and then continues by simply copying the remaining output of $S$.
\end{proof}


\subsubsection*{The strategy construction}



Finally, we explain how to construct $f_\tra$ such that (Inv0)--(Inv3) are ensured. 

The initial memory state is $[(q_0, \varepsilon, q_0^\dom, \varepsilon, q_0^\dom), (\varepsilon,\emptyset)]$. Then (Inv0)--(Inv3) are all satisfied:
\begin{itemize}
\item (Inv0) obviously holds.
\item (Inv1) holds because $q_0^\dom$ is not in $F_\dom$ because each word accepted by $A_\dom$ has to end with $\dashv$.
\item Since $R_{q_0}^\varepsilon = R_\tra$ and by assumption there is a sequential uniformizer for $R_\tra$, (Inv2) is satisfied.
\item (Inv3) is obviously satisfied by choosing $w = \varepsilon$ (because pumping the empty word results again in the empty word). 
\end{itemize}


Let $[(p,\rho,d',\xi,d);(u,M)]$ be the current memory state, $(p,\rho\xi,d)$ be the current position of the play, and assume that (Inv0)--(Inv3) are satisfied. Let $a \in \Sigmaend$ be the next move of Input leading to $(p,\rho\xi,d,a)$.

We now describe how $f_\tra$ selects the next moves of Output leading again to an Input vertex, and updates the memory. Later we verify that the invariant holds at the new Input vertex reached by the moves. For all cases, let $d_a = \delta_\dom(d,a)$.

\begin{enumerate}[(a)]
%\item If $p \in \Qin$, then $\rho\xi = \varepsilon$, $d' = d$, and $u=\varepsilon$. The only available move is (Out0), leading to $(p_1,\varepsilon,d_1)$ with $p_1 = \delta(p,a)$ and $d_1 = \delta_\dom(d,a)$. We update the memory to $[(p_1,\varepsilon,d_1,\varepsilon,d_1);(\varepsilon,\emptyset)]$. 
%
%for $p \in \Qout$ we show how to select the next move of Output such that the invariant is preserved. 
%\item If $|\rho| < K$ (and thus $\xi = u = x\varepsilon$, $d=d'$), then $f_T$ plays move (Out1) to $(p,\rho \circ \tau_a,d_1)$ with $d_1 = \delta_\dom(d,a)$, and updates the memory to $[(p,\rho,d_1,\varepsilon,d_1),(\varepsilon,\emptyset)]$.
\item Assume there is a $(p,\rho)$-uniformizer $S$ with $S(wa) \not= \varepsilon$ for all $w \in \Pump{|S|!}{(u,M)}$. Then the conditions of Lemma~\ref{lem:propagate-invariant} are satisfied. Let $q \in Q$ be the state with the properties from Lemma~\ref{lem:propagate-invariant}.

Let $w \in \Pump{|S|!}{(u,M)}$ such that $S(w) = \varepsilon$. The existence of $w$ is ensured by (Inv3) for the current node. 

We distinguish two cases depending on whether $a = \dashv$ or not.
  \begin{enumerate}[(1)]
  \item If $a \not= \dashv$, then play (Out2) with $v_{p,\rho,q}$, leading to vertex $(q,\xi,d,a)$, followed by the move (Out1) leading to $(q,\xi \circ \tau_a,d_a)$. 

Update the memory to $[(q,\xi \circ \tau_a,d_a,\varepsilon,d_a);(\varepsilon,\emptyset)]$.
  \item Assume $a = \dashv$ and $d_\dashv \in F_\dom$ (meaning that Input has played a string in the domain of $R_\tra$). In this case, the properties of $q$ are 
$\Lout(p,\rho,q) \not= \emptyset$ and $\dom(R_q^{\xi \circ \tau_\dashv}) = L(A_\dom,d_\dashv)$. Since  $L(A_\dom,d_\dashv) = \{\varepsilon\}$, the latter property implies that there is $r \in F$ with $\Lout(q,\xi \circ \tau_\dashv,r) \not= \emptyset$. So there must be $q'$ such that $\Lout(q,\xi,q') \not= \emptyset$ and $\Lout(q',\tau_\dashv,r) \not= \emptyset$.

Then $f_\tra$ plays (Out2) with $v_{p,\rho\xi,q'}$, leading to vertex $(q',\varepsilon,d,\dashv)$, followed by (Out0) with $v_{q',\tau_\dashv,r}$, leading to $(r,\varepsilon,d_\dashv)$. 

Update the memory to $[(r,\varepsilon,d_\dashv,\varepsilon,d_\dashv));(\varepsilon,\emptyset)]$.
  \end{enumerate}
\item Not case (a), and $\xi$ is not saturated. Then make the move (Out1) to $(p,\rho\xi \circ \tau_a,d_a)$.

Update the memory to $[(p,\rho,d',\xi \circ \tau_a,d_a);(ua,M)]$

This move is possible because $\xi = K$ would imply that $\xi$ is saturated  (Lemma~\ref{lem:length-saturated}).

\item Not case (a), and $\xi$ is saturated. Then there is a saturation witness $\xi = \xi_1\xi_2\xi_3$ with $\xi_3 = \varepsilon$. In particular, $M_3 = \emptyset$ for the  corresponding decomposition $(u,M) = (u_1,M_1)(u_2,M_2)(u_3,M_3)$ of $(u,M)$.
This means that $\xi_1\xi_2\xi_3 = \xi_1\xi_2$ is a saturation witness for $(u,M)$  as in Definition~\ref{def:safe-pump-word}. Then make the move (Out3) to $(p,\rho\xi_1\reduce{\xi_2},d,a)$ and update the memory to $[(p,\rho,d',\xi_1\reduce{\xi_2},d);(u,M')]$ with $M' = M \cup \{(|u_1|+1,|u_1|+|u_2|)\}$.
\end{enumerate}

\begin{lemma} \label{lem:invariant-preserved}
The strategy $f_T$ satisfies (Inv0)--(Inv3).
\end{lemma}
\begin{proof}
Most of the properties are obvious from the construction of the move:
\begin{itemize}
\item (Inv0) describes simple properties that directly follow from the construction of the new memory states. As only case we mention (Inv0)(iv). This follows from the fact that the move of type (Out3) is always applied when $\xi$ is saturated. This means if a new edge can be added to $(u,M)$ then it must involve the last letter that was added to $u$. Otherwise, the edge could have been added in a previous move.

\item (Inv1) clearly holds after (a)(2) by construction of the move. Furthermore, this is the only move after which the state of $A_\dom$ is in $F_\dom$.

\item (Inv2) holds after (b) and (c) because $p,\rho$, and $d'$ do not change. It holds after (a)(1) by Lemma~\ref{lem:propagate-invariant}. After (a)(2) the state of $A_\dom$ is in $F_\dom$ and hence (Inv2) is trivially satisfied.

\item (Inv3) is trivially satisfied after (a)(1) and (a)(2) because the new pump-word is $(\varepsilon,\emptyset)$. (Inv3) also holds after (b) because the new pump-word is $(ua,M)$ and the negation of (a) is exactly (Inv3) for $(ua,M)$. (Inv3) after (c) requires some more work, and is shown below.
\end{itemize}
We need to show that (Inv3) is preserved after an application of case (c) in the strategy description. So we need to show that for every $(p,\rho)$-uniformizer $S$ there is $w \in \Pump{|S|!}{(u,M')}$ such that $S(w) = \varepsilon$, where $M'$ extends $M$ by the new edge as defined in case (c).

Toward a contradiction, assume that there is $(p,\rho)$-uniformizer $S$ such that $S(w) = \varepsilon$ for all $w \in \Pump{|S|!}{(u,M')}$. We show that then there also exists a $(p,\rho)$-uniformizer $S'$ such that $S(w) = \varepsilon$ for all $w \in \Pump{|S'|!}{(u,M)}$, contradicting the assumption that (Inv3) holds for $(u,M)$. 

We construct $S'$ such that $|S'| \ge |S|$ and $S(w) = \varepsilon$ for all $w \in \Pump{|S|!}{(u,M)}$, which then implies $S(w) = \varepsilon$ for all $w \in \Pump{|S'|!}{(u,M)}$.

Let $\xi = \xi_1\xi_2\xi_3$ and $(u,M) = (u_1,M_1)(u_2,M_2)(u_3,M_3)$ be as in case (c). Recall that $\xi_3 = \varepsilon$ and thus $u_3 = \varepsilon$,  $\xi = \xi_1\xi_2$, and $(u,M) = (u_1,M_1)(u_2,M_2)$
%Words in $\Pump{|S|!}{(u,M')}$ are thus of the form $w_1(w_2)^\ell$ with  $w_1 \in \Pump{|S|!}{(u_1,M_1)}$ and $w_2 \in \Pump{|S|!}{(u_2,M_2)}$.

We describe how $S'$ works in two phases. We do not provide a formal definition of $S'$ because it should be clear that the description below can be implemented by a sequential finite state transducer.
\begin{itemize}
\item In the first phase, $S'$ mimics  $S$ on the input, while at the same time simulating an automaton for $\Pump{|S|!}{(u_1,M_1)}$. If during this phase $S$ produces output, $S'$ simply continues to mimic $S$ and cancels all other activities (recall that the goal is construct a transducer $S'$ that produces output on all strings from $\Pump{|S|!}{(u,M)}$; so if $S$ produces output we are done for this input string).

If $S'$ detects that $w_1 \in \Pump{|S|!}{(u_1,M_1)}$ has been read (and no output has been produced), jump to the next phase.

\item Let $s_1$ be the state of $S$ with $S:s_0 \xrightarrow{w_1/\varepsilon} s$ (which is reached during the simulation of $S$ in the first phase). Fix some $w_2 \in \Pump{|S|!}{(u_2,M_2)}$, e.g., the shortest word in this set. Let $h \ge 0$ be maximal such that starting from $s_1$, $S$ does not produce any output on $(w_2)^h$. Note that there exists a maximal such $h$ because $S$ will produce output for $|S|!$ repetitions of $w_2$. So the situation is now as follows:
\[
S: s_0 \xrightarrow{w_1 / \varepsilon} s_1 \xrightarrow{(w_2)^h / \varepsilon} s_1'
\]

In the second phase, $S'$ continues the simulation of $S$ but now from state $s_1'$. If the first output in this simulation of $S$ is produced, it is of the form $yz$ with $y \in \Lout(p,\rho,q)$ for some state $q$. Then, $S'$ outputs $y$ and jumps to the third phase.
\item The current situation can be depicted as follows, where the second line only indicates the part of $S'$ that simulates $S$:
\[
  \begin{array}{l}
S: s_0 \xrightarrow{w_1 / \varepsilon} s_1 \xrightarrow{(w_2)^h / \varepsilon} s_1' \xrightarrow{w'/yz} s_2 \\    
S': s_0 \xrightarrow{w_1 / \varepsilon} s_1 \leadsto s_1' \xrightarrow{w'/y} s_2
  \end{array}
\] 
Note that the actual input is $w_1w'$, and that $(w_2)^h$ has only virtually be inserted in the computation of $S$.

For the third phase, let $L_{\text{Pump},{s_1}'}$ be the set of all $\hat{w} \in \Pump{|S|!}{(u_1,M_1),(u_2,M_2)^h}$ with $S: s_0 \xrightarrow{\hat{w}/\varepsilon} s_1'$. Note that $w_1(w_2)^h$ is such a word, and that $L_{\text{Pump},{s_1}'}$ is regular.

In the third phase, $S'$ continues the simulation of $S$ from $s_2$ but without producing output. Instead, it waits until the output that $S$ would have produced, including the pending $z$ from the previous transition, contains a prefix $\hat{v} \in \Lout(q,\rho_{\hat{w}},r)$ for some $r$ and some $\hat{w} \in L_{\text{Pump},{s_1}'}$ such that $\Lout(q,\xi_1(\xi_2)^h,r) \not= \emptyset$. If such a prefix $\hat{v}$ is reached, then $S'$ outputs instead a word $v_1 \in \Lout(q,\xi_1,r)$, which exists because $P_{\xi_1} = P_{\xi_1}P_{\xi_2} \cdots P_{\xi_2}$. And after that, $S'$ just copies the output of $S$.
\end{itemize}


We need to argue that $S'$ is a $(p,\rho)$-uniformizer with the desired property, and  for the third phase, that the output of $S$ contains such a prefix $\hat{v}$ that can be substituted by $v_1 \in \Lout(q,\xi_1(\xi_2)^h,r)$.

For this purpose, let $x$ be an input that takes $S$ from $s_2$ into a final state $s_3$, and let $v$ be the corresponding output. The whole computation of $S$ that is used in the description above looks as follows:
\[
S: s_0 \xrightarrow{w_1 / \varepsilon} s_1 \xrightarrow{(w_2)^h / \varepsilon} s_1' \xrightarrow{w'/yz} s_2 \xrightarrow{x/v} s_3    
\]
We note that by definition of $R_\rho^p$, the pair $(w_1(w_2)^hw'x,zv)$ is accepted by $\tra$ from state $q$. Now assume that $zv = \hat{v}v'$ has a prefix $\hat{v}$ as described in the third phase. Then we can replace $w_1(w_2)^h$ in the above computations of $S$ by $\hat{w}$:
\[
S: s_0 \xrightarrow{\hat{w} / \varepsilon} s_1' \xrightarrow{w'/yz} s_2 \xrightarrow{x/v} s_3    
\]
and we thus know that $(\hat{w}w'x,\hat{v}v')$ is accepted by $T$ from $q$, and furthermore $\delta^*(q,\hat{w},\hat{v}) = (r,\varepsilon,\varepsilon)$ (for $r$ as in the third phase). By the choice of $v_1 \in \Lout(q,\xi_1,r)$ and the fact that $w_1$ is compatible with $\xi_1$, we obtain that $\delta^*(q,w_1,v_1) = (r,\varepsilon,\varepsilon)$.

The computation of $S'$ can be sketched  as follows (again only showing the states of the simulation of $S$ inside $S'$):
\[
S': s_0 \xrightarrow{w_1 / \varepsilon} s_1 \leadsto s_1' \xrightarrow{w'/y} s_2  \xrightarrow{x/v_1v'} s_3 
\] 
Since $\delta^*(q,w_1,v_1) = (r,\varepsilon,\varepsilon)$, we obtain that $(w_1w'x,v_1v')$ is accepted by $\tra$ from $q$. Hence $S'$ is indeed a $(p,\rho)$-uniformizer.

It remains to prove the existence of the prefix $v_1$ in the output $zv$.
Let us verify by applying  Lemma~\ref{lem:output-large-pumping} that the output must contain such a prefix.



Because the pumping factors for $w_1$ and $w_2$ are at least $|S|!$, one can safely pump the factors further by multiples of $|S|!$ without $S$ noticing the difference. Hence, for each $k$ one can find some $\hat{w} \in \Pump{k}{(u_1,M_1)(u_2,M_2)^h}$ with $S:s_0 \xrightarrow{\hat{w}/\varepsilon} s_1'$.
Thus, there is a prefix $v'$ of $zv$ and some  $\hat{w} \in \Pump{3|v'|}{(u_1,M_1)(u_2,M_2)^h}$ with $v' \in \Lout(q,\rho_{\hat{w}},r)$ for a state $r$. Then Lemma~\ref{lem:output-large-pumping} yields that $\Lout(q,\xi_1(\xi_2)^h,r) \not= \emptyset$.
\end{proof}

Lemma~\ref{lem:drat-uniformizer-to-strategy} now follows from
Lemma~\ref{lem:invariant-implies-winning} and
Lemma~\ref{lem:invariant-preserved}.

